Is Pseudo-Lidar needed for Monocular 3D Object detection?

Recent progress in 3D object detection from single images leverages monocular depth estimation as a way to produce 3D pointclouds, turning cameras into pseudo-lidar sensors. These two-stage detectors improve with the accuracy of the intermediate depth estimation network, which can itself be improved without manual labels via large-scale self-supervised learning. However, they tend to suffer from overfitting more than end-to-end methods, are more complex, and the gap with similar lidar-based detectors remains significant. In this work, we propose an end-to-end, single stage, monocular 3D object detector, DD3D, that can benefit from depth pre-training like pseudo-lidar methods, but without their limitations. Our architecture is designed for effective information transfer between depth estimation and 3D detection, allowing us to scale with the amount of unlabeled pre-training data. Our method achieves state-of-the-art results on two challenging benchmarks, with 16.34% and 9.28% AP for Cars and Pedestrians (respectively) on the KITTI-3D benchmark, and 41.5% mAP on NuScenes.

==> sections/abstract.tex <==


Recent progress in 3D object detection from single images has effectively leveraged monocular depth estimation as a way to produce 3D point clouds, turning cameras into pseudo-lidar sensors. These two-stage detectors improve with the accuracy of the intermediate depth estimation network, which can itself be improved without manual labels via large-scale pre-training. However, they tend to suffer from overfitting more than end-to-end methods, are more complex, and the gap with lidar-based detectors remains significant.
In this work, we propose an end-to-end, single stage, monocular 3D object detector, DD3D, that can benefit from depth pre-training more effectively than pseudo-lidar methods, but without their limitations.
Our architecture is designed for effective information transfer between depth estimation and 3D detection, allowing us to scale with the amount of unlabeled depth pre-training data.
Our method achieves state-of-the-art results on two challenging benchmarks, with $\textbf{16.34\%}$ and $\textbf{9.28\%}$ AP for ``Car'' and ``Pedestrian'' in KITTI3D benchmark.  
%with improvements of up to $80\%$ on pedestrians.


% We aims at leveraging monocular depth to improve monocular 3D object detection. Related work has shown that depth from monocular images can be used to improve 3D object detection. However, the gap to methods that rely on Lidar data as input is still significant. Our goal is to show that this gap can be partially overcome by using increasing amounts of data to pretrain the depth estimation network. Our hypothesis is, unlike standard pretraining / transfer strategies (e.g. ImageNet pretraining), 3D detection requires a pretraining scheme deliberately focused on learning good depth representation. We assume the availability of a large corpus of images paired with Lidar information, which we use to pretrain networks that predict per-pixel depth given an RGB image as input. We show that the pretrained depth networks are useful for two approaches for monocular 3D detection; FCOS-3D, a novel extension of a standard 2D detector, and Patchnet, a pseudo-lidar approach that directly consumes the output of monocular depth estimation. Further, we investigate ways of fine-tuning or adapting the pretrained monodepth network, with the aim of deploying it on a much smaller target dataset for the task of monocular 3D object detection. We aim to answer the following two questions: does supervised pretraining of the depth network (i.e. using Lidar as supervision) improve monocular 3D object detection? What are critical design choices in pretraining / fine-tune protocol and 3D detector architectures for good transfer? Finally, we show that our models achieve state-of-the-art performance on KITTI3D, Nuscenes, and Cityscapes 3D.


%Recent studies on monocular 3D detection showed that the major culprit for the large gap between Lidar-based methods and monocular methods is imprecise depth estimation from a single image. In this work, we further explore the correlation between monocular depth estimation and 3D detection by linking the best recipes of monocular depth estimation with 3D detection. As a result, we identify two effective methods to maximize the use of multimodal data: supervised pretraining on depth prediction using a large set of image-pointcloud pairs, and RoI-based depth prediction while finetuning. We show the efficacy of both approaches using two leading paradigms for monocular 3D detection: Pseudo-Lidar approach and single-stage 3D detectors. In addition, we propose a modified depth estimation metric that better reflects its transferability to 3D detection, and a novel single-stage 3D detection architecture that is extensible to a depth predictor. Finally, we demonstrate our approach on three different 3D detection benchmarks, contributing significant improvements especially on rare categories in long-tail distributed data.



% Recent studies on monocular 3D detection have shown that the major culprit for the large gap between Lidar-based and monocular methods is imprecise depth estimation from a single image. Attempts to use point-clouds from active sensors to close this gap were mainly pursued via Pseudo-Lidar based methods. In this work, we explore the possibility of using ground-truth point-clouds at training time to improve end-to-end 3D detectors. As a result, we show that supervised network pre-training on the task of depth estimation significantly improves 3D detection accuracy. We present a thorough analysis on the efficacy of depth pre-training using controlled experiments and a large-scale multimodal data. We also introduce a single-stage fully convolutional architecture 3D detection architecture, FCOS-3D,  designed for effective information transfer between depth estimation and 3D detection. Our experiments indicate that depth pre-training is a superior alternative to standard pre-training strategies, improving generalization across rare object categories in long-tail distributed data, and allowing for the training of larger networks. With no bells and whistles, we report state-of-the-art results on three different 3D detection benchmarks: KITTI 3D, nuScenes, and Cityscapes 3D. 

%to maximize the use of multimodal data: supervised pretraining on depth prediction using a large set of image-pointcloud pairs, and RoI-based depth prediction while finetuning. We show the efficacy of both approaches using two leading paradigms for monocular 3D detection: Pseudo-Lidar approach and single-stage 3D detectors. In addition, we propose a modified depth estimation metric that better reflects its transferability to 3D detection, and a novel single-stage 3D detection architecture that is extensible to a depth predictor. Finally, we demonstrate our approach on three different 3D detection benchmarks, contributing significant improvements especially on rare categories in long-tail distributed data.

%Inferring depth from a single image is inherently an ill-posed problem, with monocular 3D detection methods performing significantly worse than their LiDAR counterparts. We investigate the tasks of monocular depth estimation and 3D detection, establishing a positive correlation. Building on the Pseudo-Lidar detection paradigm, we quantify and correlate depth quality and detection accuracy. We propose a modified depth estimation metric that better explains the link between depth and 3D detection performance. We also test our hypothesis on single-stage detectors: we propose a novel 3D detection architecture (FCOS-3D) that jointly outputs dense depth and 3D object boxes, and show that depth pretraining significantly surpasses standard pretraining strategies (e.g. using COCO) for 3D detection. We show that depth pretraining especially improves generalizability in detecting rare classes, for the long-tail distributed data of driving scenes.  We also show that by attending to relevant regions in the scene (i.e. containing objects of interest) we further improve depth estimation performance, leading to better monocular 3D detection. 

==> sections/conclusion.tex <==
We proposed \textit{DD3D}, an end-to-end single-stage end 3D object detector that can leverage supervised depth estimation as an auxiliary task during the pre-training stage. We showed that the downstream task performance (i.e. 3D detection) consistently improves as the amount of raw unlabelled image and point cloud data increases, a trend that we also observed when using Pseudo-Lidar (PL) detectors. Unlike PL methods, our detector is simpler (single stage), does not require target dataset adaptation of the depth estimator, and generalizes better. 

==> sections/experiments.tex <==


\subsection{Datasets}

\noindent\textbf{KITTI-3D~\cite{geiger2012we}.} The KITTI 3D detection dataset consists of $7481$ images used for training, and $7518$ images used as the official \emph{test} set. We follow the standard protocol of further splitting the training set into $3712$ and $3769$ images \cite{}, and denote them respectively by \emph{train} and \emph{val}. We perform all ablative analysis in Sec.~\ref{subsec:3d_detection} by training on the \emph{train} set and evaluating on the \emph{val} set. The standard metrics of the KITTI benchmark consist of per-class average precision (\emph{AP}) computed with thresholds on intersection-over-union (\emph{IoU}) of 3D boxes and Bird-Eye-View (2D) boxes. In order to evaluate multiclass detectors in Sec.~\ref{subsec:3d_detection}, we additionally use mean average precision (\emph{mAP}) by computing the average of per-class APs, following other recently introduced datasets \cite{caesar2020nuscenes, gahlert2020cityscapes}.  When reporting results on the benchmark, we train on combined set of \emph{train} and \emph{val}, and perform cross-validation with 80/20 splits.

\noindent\textbf{KITTI-Depth~\cite{geiger2013vision}.} The standard training protocol of monocular depth estimation networks is to use the train/val/test splits proposed by Eigen et al.~\cite{eigen2014depth}. However, as described in ~\cite{simonelli2020demystifying}, up to a third of Eigen train images overlap with KITTI 3D images, leading to biased PL results. To avoid overfitting the PL depth on KITTI3D images, we generate a new split by removing Eigen train images that overlap (spatially within 50 meters) with the KITTI3D images. We denote this split by \textit{Eigen clean} and emphasize that for 3D detection our depth networks are finetuned on Eigen clean and \textbf{not on} Eigen train, as has been the standard practice until recently~\cite{simonelli2020demystifying}. 

% \noindent\textbf{CityScapes3D~\cite{gahlert2020cityscapes}.} The CityScapes3D dataset consists of $5000$ images of urban scenes, split into $2975$ images for training, $500$ for validating, and $1525$ for testing. It is tailored for monocular 3D detection, in that the ground-truth 3D bounding box annotations are obtained using stereo imagery, thus avoiding annotation artifacts due to parallax and synchronization error with respect to the Lidar sensor. The detection benchmark requires to report 3D bounding boxes of 6 vehicle types. The evaluation metric, \emph{mean detection score} (\emph{mDS}), is computed as the average of four depth-dependent metrics measuring errors in predicted center distance, orientation, and size, weighted by a 2D detection metric (\emph{AP}).

\noindent\textbf{nuScenes~\cite{caesar2020nuscenes}.} The nuScenes dataset consists of $1000$ multimodal videos with full $360$-degree field of view, capturing urban areas of Boston and Singapore from 6 cameras and Lidar / Radar devices. The videos are split into $700$ for training, $150$ for validating, and $150$ for testing. The 3D detection benchmark requires to report 3D bounding boxes of 10 object classes over 2Hz-sampled video frames of 360-degree view. The evaluation metric, \emph{nuScenes detection score} (\emph{NDS}), is computed by combining the detection accuracy (\emph{mAP}) computed over four different thresholds on center distance with five true-positive metrics. Among them, we only consider the three metrics that concerns 3D detection, i.e. \emph{ATE}, \emph{ASE}, and \emph{AOE}. To generate our test submissions, we use test-time augmentation by resizing test images by factors between 70\% and 130\%.

\noindent\textbf{CityScapes3D~\cite{gahlert2020cityscapes}.} The CityScapes3D dataset consists of $5000$ images of urban scenes, split into $2975$ images for training, $500$ for validating, and $1525$ for testing. We described in detail the metrics reported as well as present our results in the supplementary. 

% \noindent\textbf{Depth pretraining.} To pretrain our models, we build a large-scale internal dataset that contains monocular videos and accurate ground-truth depth captured from high-resolution Lidar devices across a full 360-degree field of view. It pictures urba\ref{table:pretraining_depth_vs_detection}n scenes in various cities of US and Japan. We randomly subsample $1K$, $5K$, $10K$, and $25K$ videos (10 seconds each), and refer to these datasets as \textbf{Pretrain-[1k, 5k, 10k, 25k]}, respectively.

% \noindent\textbf{Pretraining.}
% To quantify the effect of pretraining we utilize an internal dataset consisting of image and LiDAR pairs. The complete dataset consists of 25K scenes, each scene being captured with a frequency of $10Hz$ over $10$ seconds, for a total of 25M image + LiDAR pairs. We randomly subsample 1K, 5K and 10K scenes from the complete scene set, and generate a total of 4 pretraining splits (including the complete dataset); for brevity, we will refer to these splits as \textbf{1K}, \textbf{5K}, \textbf{10K} and \textbf{25K} whenever appropriate. Importantly, the downsampled splits contain fewer images as well as less diversity, as we downsample from the scene set and not from the image set. 

\subsection{Implementation}
\label{implementation}
\textbf{DD3D.} We use two bottom-up architectures for FPN, V2-99~\cite{lee2019centermask} and DLA-34~\cite{yu2018deep}. Unless noted otherwise, results reported on KITTI3D benchmark use V2-99 backbone, and results reported nuScenes uses DLA-34 backbone. The $\sigma_l$ and $\mu_l$ are initialized using depth statistics of objects that are associated with each FPN level, and $(W_0, H_0, D_0)$ are set as averages of per-class dimensions available from training data. The returned 3D bounding boxes from network is filtered using non-maxima suppression using intersection-over-union criteria on 2D bounding boxes, but using 3D confidence scores to rank the detected objects.

\textbf{PL.} When training PackNet~\cite{packnet} we use a batch size of 4 and a learning rate of $5e^{-5}$. We train until convergence on each pre-training split (more details in the supplementary), and for 5 epochs over the KITTI \textit{Eigen clean} split during fine-tuning. The PL 3D detector is trained with a learning rate of $1e^{-4}$ for 100 epochs, decayed by $0.1$ after 40 and 80 epochs, respectively. For both networks we use the Adam~\cite{loshchilov2017decoupled} optimizer with $\beta_1=0.9$ and $\beta_2=0.999$. Both methods are implemented using Pytorch~\cite{paszke2017automatic} and trained on 8 V100 GPUs.

%All our methods are implemented using Pytorch~\cite{paszke2017automatic} and trained on 8 V100 GPUs. For completeness we provide details on the FPN and 2D detection heads in the supplementary. We use two bottom-up architectures for FPN, DLA-34~\cite{yu2018deep} and V2-99~\cite{lee2019centermask}. The results reported on KITTI3D benchmark used V2-99 backbone, and all other experiments including ablative analysis use DLA-34. The $\sigma_l$ and $\mu_l$ are initialized using depth statistics of objects that are associated with each FPN level, and $(W_0, H_0, D_0)$ are set as averages of per-class dimensions available from training data. The returned 3D bounding boxes from network is filtered using non-maxima suppression using intersection-over-union criteria on 2D bounding boxes, but using 3D confidence scores to rank the detected objects. When training PackNet~\cite{packnet} we use a batch size of 4 and a learning rate of $5e^{-5}$. We train until convergence on each pre-training split (more details in the supplementary), and for 5 epochs over the KITTI \textit{Eigen clean} split during fine-tuning. The PL 3D detector is trained with a learning rate of $1e^{-4}$ for 100 epochs, decayed by $0.1$ after 40 and 80 epochs, respectively. For both networks we use the Adam~\cite{loshchilov2017decoupled} optimizer with $\beta_1=0.9$ and $\beta_2=0.999$. 

% \noindent\textbf{Depth pretraining.} 

% \noindent\textbf{FCOS-3D.}

%\subsection{Depth estimation.}
 

%\noindent\textbf{Pretraining.}
%To quantify the effect of depth quality we pretrain our depth estimation networks on a large internal dataset consisting of image and LiDAR pairs. The complete dataset consists of 25K scenes, each scene being captured with a frequency of $10Hz$ over $10$ seconds, for a total of 25M image + LiDAR pairs. We randomly subsample 1K, 5K and 10K scenes from the complete scene set, and generate a total of 4 pretraining splits (including the complete dataset); for brevity, we will refer to these splits as \textbf{1K}, \textbf{5K}, \textbf{10K} and \textbf{25K} whenever appropriate. Importantly, the downsampled splits contain fewer images as well as less diversity, as we downsample from the scene set and not from the image set. We use the generated splits for pre-training the depth networks, and we perform experiments that estimate depth quality vs. 3D detection performance at each pretraining level. We describe the pretraining protocol in detail in the supplementary. 

% and mention that we ensured that each model is trained to convergence. 


% \subsection{FCOS-3D}
% \textbf{Pretraining backbone}
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=1.0\columnwidth]{figures/fcos3d_backbone_pretrained.png}
% \end{figure}


==> sections/introduction.tex <==

% structure:
% task: what and why
% sota: brief + excite / praise (not dis)
% flaw in sota + why should we care + why hard / no current sol (use example)
% idea: main intuition (no details)
% proof it works / results

% task
Detecting and accurately localizing objects in 3D space is crucial for many applications, including robotics.
% Traditional methods use range sensor measurements (e.g. from LiDAR) to actively perceive the underlying scene geometry and relate them to object shape, position, and class~\cite{qi2018frustum}. Recently, CNN-based methods have shown that RGB images without associated depth measurements can be used to directly regress object properties in 3D space~\cite{kehl2017ssd,simonelli2019disentangling}.
Hence, monocular 3D detection is an active research area~\cite{manhardt2019roi,simonelli2019disentangling,liu2020smoke,you2019pseudo}, owing to its potentially wide-ranging impact and the ubiquity of cameras.
% sota: brief + excite / praise (not dis)
Leveraging exciting recent progress in depth estimation~\cite{eigen2014depth, dorncvpr, godard2018digging2, packnet,lee2019big}, pseudo-lidar detectors~\cite{you2019pseudo,ma2020rethinking,simonelli2019disentangling} first use a pretrained depth network to compute an intermediate point cloud representation, which is then fed to a second 3D detection network. The strength of pseudo-lidar methods is that they monotonically improve with depth estimation quality, e.g., thanks to large scale training of the depth network on raw data.
% flaw in sota + why should we care + why hard / no current sol (use example)
% PL methods are good but rather complicated + overfit.
However, regressing depth from single images is inherently an ill-posed problem. Consequently, errors in depth estimation account for the major part of the gap between pseudo-lidar and lidar-based detectors, a problem compounded by generalization issues that are not fully understood yet~\cite{simonelli2020demystifying}.
% e2e not solved it either
Simpler end-to-end monocular 3D detectors~\cite{brazil2019m3d,liu2020smoke} seem like a promising alternative, although they do not enjoy the same scalability benefits of unsupervised pre-training due to their single stage nature.

\begin{figure}[t!]
\centering
\vspace*{-3mm}
\hspace*{-7mm}
\includegraphics[width=0.55\textwidth]{figures/teaser_figure.png}
\vspace*{-3mm}
\caption{\textbf{FCOS-3D}: We introduce a single-stage 3D object detector that combines the best of both pseudo-lidar methods (scaling with depth pre-training) and end-to-end methods (simplicity and generalization performance). Our detector features a simple training protocol of depth pre-training (\textcolor{green}{green}) and detection fine-tuning (\textcolor{red}{red}), compared to pseudo-lidar methods that require an additional depth fine-tuning step (\textcolor{blue}{blue}) and tend to overfit to depth errors.}
\label{fig:teaser}
\vspace*{-3mm}
\end{figure}


% idea: main intuition (no details)
In this work,  we aim to get the best of both worlds: the scalability of pseudo-lidar with raw data and the simplicity and generalization performance of end-to-end 3d detectors. To this end, our \textbf{main contribution} is a novel fully convolutional single-stage 3D detection architecture, \textit{FCOS-3D}, that can effectively leverage monocular depth estimation for pre-training.
% proof it works / results
Using a large corpus of unlabeled raw data, we show that FCOS-3D scales similarly to pseudo-lidar methods, and that depth pre-training improves upon pre-training on large labeled 2D detection datasets like COCO~\cite{lin2014microsoft}, even with the same amount of data.
Our method sets a new state of the art for the task of monocular 3D detection on KITTI3D~\cite{geiger2012we} and NuScenes~\cite{caesar2020nuscenes}. We also discover a side-benefit of large-scale unsupervised depth pre-training: significant improvement on rare classes with only few 3D labels (e.g., $80\%$ relative improvements on pedestrians in KITTI3D and nuScenes).

% Cityscapes3D~\cite{gahlert2020cityscapes},
% below is redundant 
%To summarize: our main contribution is FCOS-3D, a novel single stage end-to-end 3D detector, aimed at regressing depth-aware features by effectively combining monocular depth estimation and 3D object detection. For our second contribution, we show that raw, unlabelled data in the form of synchronized image - point cloud pairs, can be used to improve the down-stream task of 3D object detection, with a surprisingly clear correlation between the two tasks.


% Detecting and accurately localizing objects in 3D space is crucial for autonomous mobile operation. Traditional methods use range sensor measurements (e.g. from LiDAR) as proxies for the underlying scene geometry and relate them to object shape, position, and class~\cite{qi2018frustum}. Recently, CNN-based methods have shown that RGB images without associated depth measurements can be used to directly regress object properties in 3D space~\cite{kehl2017ssd,simonelli2019disentangling}. Monocular 3D detection has attracted a great deal of attention in the community, owing to its potentially wide ranging impact: cameras are ubiquitous, cheap, and provide dense signal. However, regressing depth from single images is inherently an ill-posed problem. Accordingly, the error in depth estimation accounts for the major culprit for the large gap between RGB-based methods and Lidar-based methods ~\cite{simonelli2020demystifying}. To address this gap, a recent line of works \cite{} promoted \emph{Pseudo-Lidar} (PL) methods as an approach for using imagery coupled with point-cloud data. Despite the success in KITTI3D benchmark, much of the gain in accuracy turned out to be attributable to the bias in evaluation protocol ~\cite{simonelli2020demystifying}.  %However, a large part of gain reported by PL methods was proved to be attributable to the bias in evaluation protocol of KITTI3D benchmark \cite{simonelli2020demystifying}.

% In this work, we aim to explore how a large-scale point-cloud data can be used to improve end-to-end 3D detectors.  As a result, we show that \emph{pre-training a simple multi-task architecture using a large-scale image-Lidar data} is sufficient to outperform other approaches that requires two-stage pipeline \cite{} or handcrafted geometric prior \cite{}, \emph{with no bells and whistles.} Since we introduce no design tailored for a particular sensor configuration or object category, our approach is generalizable to multiple datasets and object categories, while still outperforming all existing approaches on commonly reported metrics, i.e. ``Car'' of KITTI3D.


% Our main contribution is following:
% \begin{itemize}
% \item We introduce a novel single-stage network architecture, \emph{FCOS-3D}, that performs 3D detection and dense depth prediction. The  architecture  is  designed  to maximize the parameter sharing between the two tasks, assuring the depth representation learned during pre-training effectively transfer to  3D  detection task.
% \item  We show that pre-training FCOS-3D using a large set of image-Lidar pairs signficantly improve the accuarcy in 3D detection. We present a thorough ablative study that shows our proposed pre-training methods on FCOS-3D 1) is a superior alternative of other pre-training tasks, 2) is \emph{scalable} -- the accuracy keep improves with large data, 3) provides generalizablity across multiple classes in long-tail distributed data, and 4) allows for training very large networks.
% \item We show that FCOS-3D pre-trained on a large set of depth data can be fine-tuned for 3D detection on multiple datasets and object categories, without making assumptions on scene geometry or sensor configuration, or training separate models per each category. In addition to ``Car'' category of KITTI3D benchmark, we also report state-of-the-art performance of three multiclass 3D detection benchmarks -- KITTI3D, nuScenes, and Cityscapes 3D.
% \end{itemize} 
% \todo{DP}{mention depth-as-major-culprit}

% As an upper bound, we compute depth and 3D detection metrics from stereo images.

%In this work, we aim to establish a correlation between depth estimation and 3D object detection from monocular images. We leverage \textit{Pseudo-Lidar (PL)} style 3D detectors, where depth regression is an intermediate task, and we achieve clear improvements in 3D detection that correlate with depth quality. To further test our hypothesis, we propose a novel fully convolutional single stage 3D detection architecture (FCOS-3D) that jointly outputs dense depth and 3D object boxes. Our results show that depth pretraining significantly surpasses COCO~\cite{lin2014microsoft} pretraining for 3D object detection. Additionally, we perform an analysis of standard depth estimation metrics employed by the community and reveal an underlying bias: depth performance on objects is significantly worse than what is reported by metrics averaged over whole scenes. We propose computing depth \textit{metrics per object}, and show a stronger \textit{correlation between depth and 3D detection performance}. We also show that by attending to relevant regions in the scene (i.e. containing objects of interest) we further improve depth estimation performance, leading to better monocular 3D detection.

% In this work, we aim to establish a correlation between depth estimation and 3D object detection from monocular images. We perform experiments with two leading approaches for monocular 3D detection: (i) \textit{Pseudo-Lidar (PL)} style methods, where depth regression is an intermediate task; and (ii) dense 3D prediction methods that output depth and 3D object boxes jointly. In both cases, we show that by \textit{pretraining the depth} component, we achieve clear improvements in 3D detection that correlate with depth quality. Our analysis of standard depth estimation metrics employed by the community reveals an underlying bias: depth performance on objects is significantly worse than what is reported by metrics averaged over whole scenes. We propose computing depth\textit{ metrics per object}, and show a stronger \textit{correlation between depth and 3D detection performance}. We also show that by attending to relevant regions in the scene (i.e. containing objects of interest) we further improve depth estimation performance, leading to better monocular 3D detection. 
    % \item We propose two methods that link the leading approaches in monocular depth estimation with effective 3D detection. 
    % \item First, we propose to use a large set of unlabeled image-pointcloud pairs to \emph{pre-train} depth estimation models. The pre-trained models are used both in PL-based models, by providing more accurate depth as inputs, and in single-stage detector, by serving as better initialization of the model. 
    % \item Second, we propose to use \emph{attention-based} depth estimation that focus on foreground region, while finetuning the model. For PL-based method, the pretrained depth network is further finetuned on target domain; for single-stage method depth estimation is used as an auxiliary task during training.
    
%For \textbf{our main contribution} we introduce \textbf{FCOS-3D} - a single-stage network architecture for 3D detection and dense depth prediction. The architecture is designed to maximize the parameter sharing between 3D detector and depth predictor, so that the depth representation learned during pre-training effectively transfer to 3D detection task.  For \textbf{our second contribution}, we propose to use a large set of unlabeled image-pointcloud pairs to \emph{pre-train} depth estimation models. The pre-trained models are used both in PL-based models, by providing more accurate depth as inputs, and in single-stage detector, by serving as better initialization of the model. We demonstrate the proposed approaches on three standard 3D detection benchmarks; KITTI 3D, CityScapes 3D, and nuScenes. We report the state-of-the-art performance on all three benchmarks, with significant improvements from the best published results to date on the rare categories.

% Our main contributions are:
% \begin{itemize}
%     % \item We introduce a simple extension of existing single-stage 2D detector architecture for 3D detector and dense depth prediction, \emph{FCOS-3D}. The architecture is designed to maximize the parameter sharing between 3D detector and depth predictor, so that the depth representation learned during pre-training effectively transfer to 3D detection task.  
%     \item We propose to use a large set of unlabeled image-pointcloud pairs to \emph{pre-train} depth estimation models. The pre-trained models are used both in PL-based models, by providing more accurate depth as inputs, and in single-stage detector, by serving as better initialization of the model. 
%     % \item We propose a novel metric for depth estimation, \todo{DP}{name-of-metrics}, that correlates better with the accuracy in 3D detection. The metric focus more on the pixels with larger depth, where typical monocular 3D detectors struggle. 
%     \item We demonstrate proposed approaches on three standard 3D detection benchmarks; KITTI 3D, CityScapes 3D, and nuScenes. We report the state-of-the-art performance on all three benchmarks, with large gaps from others on the rare categories in long-tail distribution.  
    
% \end{itemize}
 
%Our main contribution is showing a clear trend between depth quality and 3D detection performance from monocular images; we propose a modification to current depth estimation metrics that better correlates the two tasks. Our second contribution is a novel loss formulation that improves depth estimation on objects, leading to superior 3D detection performance. Our third contribution is a novel, dense one-stage network architecture (\textit{FCOS-3D}), combining depth and 3D detection in a multi-scale formulation.


% \begin{itemize}
% \item The key of robust monocular 3D detection is accurate depth prediction.
% \item Existing approaches follow the standard pretraining strategies, such as ImageNet pretraining.
% \item We show monocular 3D detection is significantly improved by leveraging depth estimation network pretrained on large-scale images paired with Lidar data.
% \end{itemize}

% Our contributions are:
% \begin{itemize}
%     \item Novel architecture: we introduce FCOS-3D, a one-stage 3D detector, that surpasses all other existing one-stage 3D detectors in accuracy (e.g. CenterNet, SMOKE), and perform on part with SOTA the two-stage detector (MonoDis).
%     \item Versatility: we show that the pretrained depth benefits two monocular 3D detection approaches that are very different in design: FCOS-3D and PatchNet.
%     \item Pretraining methodology: we investigate what are important factors in depth pretraining for good transfer to 3D detection. I.e., how much of pretrain data needed? Is it useful to focus on a certain range of depth? What are specifically important in fine-tuning for PatchNet or FCOS-3D?
%     \item We contribute state-of-the-art monocular 3D detector on KITTI3D, Nuscenes, and Cityscapes 3D. In particular, our methods significantly outperform other baselines in challenging object categories, such as pedestrians and bicycles.
% \end{itemize} 

==> sections/method.tex <==
% \input{tables/baseline_depth_detection}


% The goal of 3D object detection from monocular images is the recovery of objects in 3D space, parameterized by their 3D position, 3D shape, class and confidence. Accurately regressing object position is by far the most challenging task~\cite{manhardt2019roi,simonelli2020demystifying}.  Intuitively, monocular depth estimation and monocular object detection are linked; in this work we dive deeper and establish a clear correlation between the two. We thoroughly test our hypothesis following two leading 3D detection paradigms: (i) single stage methods~\cite{tian2019fcos,liu2020smoke} that directly regress object properties for each pixel, where we propose a novel \textit{Fully Convolutional} architecture (FCOS-3D)  that combines dense depth estimation and dense object detection; and (ii) \textit{Pseudo-Lidar} (PL) methods~\cite{you2019pseudo,vianney2019refinedmpl,qian2020end,ma2020rethinking}, where depth estimation is an intermediate task with the resulting point cloud being consumed as input by a 3D detector.

We start by introducing DD3D, an end-to-end approach to 3D object detection. We then describe the alternative Pseudo-LiDAR approach we use to compare both performance and scalability of depth pre-training.
% further introspect the correlation between monocular depth estimation and 3D object detection.

\subsection{FCOS-3D}
\input{sections/method_fcos}

\subsection{Pseudo-Lidar 3D detection}
\label{subsec:pseudo-lidar}
\input{sections/method_pl}

==> sections/method_fcos.tex <==
%\subsection{FCOS-3D}
 
\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\columnwidth]{figures/fcos3d_arch.png}
	\caption{FCOS-3D extends FCOS to perform 3D detection and dense depth prediction. As in FCOS, a shared head is applied to all levels of FPN features, but with one exception: the depth head is only applied on to the highest resolution features (i.e. $\texttt{p3}$ features).}
	\label{fig:fcos-3d}
	\vspace{-3mm}
\end{figure}



\noindent\textbf{Task.} The goal of monocular 3D detection is to generate a set of category-specific 3D bounding boxes in camera frame. In addition to an RGB image, FCOS-3D takes camera intrinsics matrix as input to account for pixel pitch.

\noindent\textbf{Architecture.} FCOS-3D is a fully convolutional single-stage network that extends~\cite{tian2019fcos} to perform 3D detection and dense depth prediction. We depict the network architecture in Figure~\ref{fig:fcos-3d}.
%It is composed of a backbone network and three \emph{subnetworks}. 
%We adopt the basic structure of FCOS.
The architecture is composed of a backbone network and three shared \emph{head} sub-networks. The backbone takes an RGB image as input, and computes convolutional features at different scales. As in \cite{tian2019fcos}, we adopt a feature pyramid network (FPN) \cite{lin2016fpn} as the backbone.

%to further process and combine the backbone features to generate per-scale feature maps.
% As in \cite{tian2019fcos}, we adopt feature pyramid network (FPN) \cite{lin2016fpn} as the backbone. Two of the three subnetworks are identical to the ones of FCOS. 

The three head networks are applied to each feature map produced by the backbone, and perform an independent prediction task. 
The classification module predicts object classification and centerness. It produces $C + 1$ real values, where $C$ is the number of object categories. The 2D box module predicts class-agnostic bounding box regression, and produces $4$ offsets from the feature location to the sides of bounding boxes. We refer the reader to ~\cite{tian2019fcos} for more details regarding the 2D detection architecture.

\noindent\textbf{3D detection head.} %In the 3D prediction, 
% Our novelty lies in the third subnetwork that performs 3D bounding box regression and dense depth prediction. 
The third head performs 3D bounding box regression and dense depth prediction. It takes FPN features as input, and applies four 2D convolutions with $3 \times 3$ kernels that generate $12$ real values for each feature location. These are decoded into 3D bounding box, 3D prediction confidence, and per-pixel depth map. The 3D box decoding is similar to \cite{simonelli2020disentangling}, except that we use a class-agnostic 3D bounding box:
\begin{itemize}
     \item $\mathbf{q} = (q_w, q_x, q_y, q_z)$ is a quaternion representation of \emph{allocentric} orientation ~\cite{manhardt2019roi, simonelli2019disentangling, liu2020smoke}. It is normalized and transformed to an egocentric orientation \cite{manhardt2019roi}.
     \item $\mathbf{o} = (\Delta_u, \Delta_v)$ are offsets from feature location to the projected 3D bounding box center, i.e. $(u_b + \Delta_u, v_b + \Delta_v$), where $(u_b, v_b)$ is the feature location.
     \item $z_c$, $z_p$ are depth predictions for 3D bounding box center and per-pixel depth. They are \emph{unnormalized} using per-level parameters (in an FPN sense) as follows:
    \begin{align}
        z &= p \cdot (\sigma_l \cdot d + \mu_l), \\
        p & = \sqrt{{\frac{1}{f_x^2}  + \frac{1}{f_y^2}}}.
    \end{align}
    $\sigma_l$ and $\mu_l$ are a learnable scaling factor and offset, maintained for each PFN level. $p$ is the \emph{pixel pitch} computed from the camera focal lengths, $f_x$ and $f_y$. This partially addresses the scale-depth ambiguity, when input images are of variable resolution (e.g. resize transformation as a form of data augmentation). $\{z_p\}$ collectively represent low-resolution versions of the dense depth map. To recover the full resolution of the dense depth map, we apply bilinear interpolation.
    \item $\mathbf{\delta} = (\delta_W, \delta_H, \delta_H)$ represents the deviation in the size of the 3D bounding box from the class-specific canonical size, i.e. $\mathbf{s} = (W_0 e^\delta_W, H_0 e^\delta_H, D_0 e^\delta_D)$
    \item $\beta_{3D}$ represents the confidence of the 3D bounding box prediction \cite{simonelli2019disentangling}. It is transformed into a probability: $p_{3D} = (1 + e^{-\beta_{3D}})^{-1}$.
\end{itemize}
Notably, we compute dense depth $z_p$ only at the lowest FPN level. This design is motivated by the observation that most of the error in 3D detection is due to inaccurate depth estimation on small objects (in pixel space), which the lowest level of the FPN is responsible for detecting.
%This is motivated by the design of FPN that each level is responsible for detecting objects of designated range of size (in pixel). During training, the $\sigma_l$ and $\mu_l$ are initialized using per-level statistics of object (centroid) depths assigned to the given level

%The FPN features are first processed by a series of $3 \times 3$ convolutions, similarly to the other two subnetworks. %The final $3 \times 3$ convolution produces $12$ real values for each feature location that are decoded into 3D bounding box, confidence for 3D prediction, and per-pixel depth map. %We parameterise the 3D predicted targets as follows:

% As in \cite{manhardt2019roi, simonelli2019disentangling}, we choose to encode 3D cuboid by a 10D vector that is composed of a unit quaternion for rotation, 3D translation, and extents. The network regresses 2D offsets of the projected 3D centroid from the given feature location, together with the associated depth. For 3D extents, the network predicts the log-scale deviation from the canonical size of the object category in meter. The rotation is decoded by simply normalizing the relevant 4D vector to achieve unit norm. 

% To address the large variance of the depth -- both centroid depth and per-pixel depth -- , we model depth in \emph{per-level} fashion. Motivated by the design of the FPN that CNN features of each level are responsible for detecting objects of given range of size (in pixel), the model maintains a learnable scaling factor, $\sigma_l$, and an offset, $\mu_l$, that are used to \emph{unnormalize} the subnetwork output from level $l$. During training, the $\sigma_l$ and $\mu_l$ are initialized using per-level statistics of object (centroid) depths assigned to the given level.

% In addition, in order to address the inherent scale-distance ambiguity while accepting input images of variable resolution, we apply additional scaling using the \emph{pixel pitch} computed from camera intrinsics. This allows for using re-size transformation as a form of data-augmentation during training, since resizing image is equivalent to scaling focal lengths. The final depth prediction is computed as following:

\noindent\textbf{Losses} We adopt the classification loss and 2D bounding box regresssion loss from FCOS \cite{tian2019fcos}:
% \begin{equation}
% \begin{split}
% \label{eq:loss_function}
% \mathcal{L}_{2D} = \mathcal{L}_{reg}(t_{x,y}, t^*_{x,y})\mathbb{1}_{c^*_{x,y}>1}\\ + \mathcal{L}_{cls}(c_{x,y},c^*_{x,y}) + \mathcal{L}_{centerness}(C_{x,y},C^*_{x,y}),
% \end{split}
% \vspace{-2mm}
% \end{equation}
\begin{equation}
\label{eq:loss_function}
\mathcal{L}_{2D} = \mathcal{L}_{reg} + \mathcal{L}_{cls} + \mathcal{L}_{centerness},
\end{equation}
where the bounding box regression $L_{reg}$ is the IOU loss~\cite{yu2016unitbox}, the classification loss $L_{cls}$ is the focal loss and the centerness regression loss $L_{centerness}$ is the binary cross entropy loss. Our 3D bounding box regressiong loss is defined as~\cite{simonelli2019disentangling,ma2020rethinking}:

\begin{equation}
\label{eq:loss_function}
L_{3D}^{bb}(B, \hat{B}) &= \frac{1}{8}||B - \hat{B}||_1
\end{equation}
% The formulation of these losses are identical to \cite{simonelli2019disentangling}. 
% we adopt the disentangledloss

In addition to the 2D and 3D losses, we adopt the self-supervised confidence loss for 3D bounding box following~\cite{simonelli2019disentangling}, which is computed as:
\begin{align}
     \hat{p}_{3D} &= e^{-\frac{1}{T} L_{3D}^{bb}(B, \hat{B})}, 
     \label{eq:confindence_loss_fcos} \\
    \mathcal{L}_{conf} &= CE(p_{3D}, \hat{p}_{3D})
\end{align}
where $B$ and $\hat{B}$ are vertices of ground-truth and predicted 3D box, and $T$ is the temperature parameter. To balance the 2D and 3D losses we follow the disentangled loss formulation proposed in~\cite{simonelli2019disentangling}.

% The disentangled loss $\mathcal{L}_{dis}$ is computed over three group of parameters; $\mathbf{q}$, $\mathbf{o}  \cup \{z_c\}$, and $\delta$. 

\noindent\textbf{Depth pre-training.}
Thanks to its dense depth head $z_p$, our FOCS-3D architecture can also be used for depth estimation, and thus pre-trained on raw camera + LiDAR data by optimizing only for that task (the other heads being initialized randomly).
In this case, we use an L1 loss between the predicted depth and the reprojected LiDAR point cloud. In practice, we found the L1 loss to be more stable than the Scale Invariant Log (SILog)~\cite{eigen2014depth} loss commonly used for supervised monocular depth estimation. 

To measure the scaling law of 3D detection performance with depth pre-training, we utilize an internal dataset consisting of synchronized and calibrated image and LiDAR scan pairs. The complete dataset consists of 25K scenes, each scene being captured with a frequency of $10Hz$ over $10$ seconds, for a total of 2.5M image + LiDAR pairs. We randomly subsample 1K, 5K, and 10K scenes from the complete scene set, and generate a total of 4 pre-training splits (including the complete dataset); for brevity, we will refer to these splits as 1K, 5K, and 10K. Importantly, the downsampled splits contain fewer images as well as less diversity, as we downsample from the set of \emph{scenes}. %, not the set of images. 

%\begin{align}
%    \mathcal{L}_{dis}(y, \hat{y}) = \frac{1}{k}\sum_{j=1}^k %L(\psi(\theta_j, \hat{\theta}_{-j}), \hat{y}),
%\end{align}
 %That is, each level of FPN maintain a pair of learnable scale and offset used to \emph{unnormalize} the network output. 



% \noindent\textbf{Dense depth.}




==> sections/method_pl.tex <==
% PL methods consist of two stages:
An alternative way to utilize a large set of image-LiDAR frames is to adopt \textit{Pseudo-Lidar (PL)} paradigm and aim to improve the depth network component using the large scale data. PL is a two-stage method: first, given an image it applies a dense depth network to predict per-pixel depth. The per-pixel depth map is transformed into the 3D point cloud using camera intrinsics, and then a pipeline similar to Lidar-based 3D detector is used to predict 3D bounding box. The modularity of PL methods enables us to quantify of role of improved depth predictors brought by a large-scale image-LiDAR data.
%To compare with DD3D and further introspect the correlation between monocular depth estimation and 3D object detection, we follow the \textit{Pseudo-Lidar (PL)} 3D detection paradigm. First, leveraging a dense depth estimator, a point cloud is computed given an input RGB image. Second, a 3D detector consumes the generated point cloud, outputting detections. The modularity of the PL pipeline implies that any depth estimation method can easily be combined with any detector that consumed point cloud data as input. Moreover, this paradigm allows easy introspection of both components, permitting us to quantify how changes in one affects performance in the other. 

% \subsubsection{Monocular depth estimation}
% \label{subsubsec:monodepth}

\noindent\textbf{Monocular depth estimation.} The aim of monocular depth estimation is to compute the depth $\hat{D} = f_D\left( I\left(p\right)\right)$ for each pixel $p \in I$. Given ground truth depth measurement $D$ (typically acquired by an external sensor, e.g. a LiDAR or RGB-D camera), we define a loss by the error between the predicted and the actual depth. We supervise our predictions using the Scale Invariant error in Logarithmic space (SILog) proposed by~\cite{eigen2014depth,lee2019big}.

\noindent\textbf{Network architecture.} In all our experiments we use the PackNet~\cite{guizilini20203d}, a state-of-the-art monocular depth prediction architecture which uses packing and unpacking blocks with 3D convolutions, allowing it to recover fine structures with high precision; moreover, PackNet has been shown to generalize better thanks to its increased capacity~\cite{guizilini20203d}.


% \noindent\textbf{Monocular depth estimation.} The aim of monocular depth estimation is the recovery of a function $f_D: I \to D$ that predicts for each pixel $p \in I$ the estimated depth $\hat{D} = f_D\left( I\left(p\right)\right)$. Given ground truth depth measurement $D$ (typically acquired by an external sensor, e.g. a LiDAR or RGB-D camera), we define a loss aimed at minimizing the error between the predicted and the actual depth. We supervise our predictions using the scale invariant error proposed by~\cite{eigen2014depth}:  

% \begin{equation} \label{eq:silog_loss}
% \small
% \mathcal{L_D}(D, \hat{D}) =
% \frac{1}{N} \sum_{d \in D} e ^2 - \frac{\lambda}{N^2} \left(\sum_{d \in D} e \right)^2
% \end{equation}

% \noindent where $e$ denotes the error in log space between the predicted and actual depth, $e = \log \hat{d} - \log d$. We follow~\cite{lee2019big} and set $\lambda=0.85$. 

% \noindent\textbf{Network architecture.} In all our experiments we use the PackNet~\cite{guizilini20203d} state-of-the-art monocular depth prediction architecture which uses packing and unpacking blocks with 3D convolutions, allowing it to recover fine structures with high precision; moreover, PackNet has been shown to generalize better thanks to its increased capacity~\cite{guizilini20203d}.


% \subsubsection{3D detection}
% \label{subsubsec:pl_3d_det}

\noindent\textbf{3D detection.} Our Pseudo-Lidar monocular 3D detector follows the method proposed by~\cite{qi2018frustum,ma2020rethinking}. Given an input image $I$, we predict dense per pixel depth which is converted to a 3D point cloud using the camera intrinsics $K$. The point cloud is concatenated with the input image, resulting in a 6D tensor encompassing pixel color values along with 3D coordinates. Leveraging an off-the-shelf 2D detector, proposal regions are identified in input images and fed to a 3D detection network that outputs bounding boxes.

\noindent{\textbf{Backbone, detection head and 3D confidence.}}
We follow~\cite{ma2020rethinking} and process each RoI with a ResNet-18~\cite{he2016deep} backbone that uses Squeeze-and-Excitation layers~\cite{hu2018squeeze}. As the RoI contains both objects as well as background pixels, the resulting features are filtered via a foreground/background mask computed based on the associated RoI depth map~\cite{ma2019accurate}. The detection head follows~\cite{ma2020rethinking} and operates in 3 distance ranges, outputting one bounding box for each range. The final output is then selected based on the mean depth of the input RoI. Following~\cite{simonelli2019disentangling,simonelli2020demystifying}, we modify the detection head to also output a 3D confidence value $\gamma$ per detection, which is linked to the 3D detection loss. More details are described in the supplementary material.

\noindent{\textbf{Loss function.}} Following~\cite{qi2018frustum} the 3D regression loss is defined as:
\begin{equation} \label{eq:3D_bbox_loss}
\small
\mathcal{L}_{3D} = \mathcal{L}_{center} +  \mathcal{L}_{size} +  \mathcal{L}_{heading} +  \mathcal{L}_{corners}
\end{equation}
We define an additional loss that links the predicted 3D confidence $\gamma$ with the 3D bounding box coordinates loss~\cite{simonelli2019disentangling} using a Binary Cross Entropy (BCE) formulation with target $\hat{\gamma}=e^{-\mathcal{L}_{corners}}$, as defined in Eq.~\ref{eq:confindence_loss_fcos}. The final PL 3D detection loss is: $\mathcal{L}_{PL} = \mathcal{L}_{3D} +  \mathcal{L}_{conf}.$

% Following~\cite{ma2020rethinking}, each RoI is processed by a 3D detection backbone network which outputs deep features. A detection head converts the features into 3D boxes. Following~\cite{simonelli2019disentangling,simonelli2020demystifying}, we modify the detection head and also output a 3D confidence value $\gamma$ per detection, which is linked to the 3D detection loss. The final PL 3D detection loss is:

% \begin{equation} \label{eq:3D_PL_loss}
% \small
% \mathcal{L}_{PL} = \mathcal{L}_{3D} +  \mathcal{L}_{conf}.
% \end{equation}

% \noindent where $\mathcal{L}_{3D}$ follows~\cite{qi2018frustum} and consists of center, size and heading regression terms. The additional loss term $\mathcal{L}_{conf}$ links the predicted 3D confidence $\gamma$ with the 3D box coordinates loss~\cite{simonelli2019disentangling} using a Binary Cross Entropy (BCE) formulation with target $\hat{\gamma}=e^{-\mathcal{L}_{corners}}$. 



==> sections/qualitative.tex <==
\begin{figure*}
\vspace{-2mm}
\centering
% [trim=left bottom right top, clip]
\subfloat{
\includegraphics[width=0.65\linewidth]{figures/000020.jpg}
\includegraphics[width=0.25\linewidth]{figures/000020_bev.jpg}
} \\ 
\subfloat{
\includegraphics[width=0.65\linewidth]{figures/000454.jpg}
\includegraphics[width=0.25\linewidth]{figures/000454_bev.jpg}
}\\

\vspace*{-2mm}
\caption{
\textbf{Qualitative results of FCOS-3D applied on the KITTI3D ~\cite{geiger2012we}.} It can detect highly occluded cars up to 75m, achieving state-of-the-art vision-based method on KITTI \emph{test}.}
\label{fig:supp_results_qualitative}
\end{figure*}

==> sections/qualitative_cs.tex <==
\begin{figure*}
\vspace{-2mm}
\centering
% [trim=left bottom right top, clip]

\subfloat{
\includegraphics[width=0.45\linewidth]{figures/cs/0065.jpg}
\includegraphics[trim=0 0 0 0,clip,width=0.45\linewidth]{figures/cs/0065_bev.jpg}
} \\ 
\subfloat{
\includegraphics[width=0.45\linewidth]{figures/cs/0079.jpg}
\includegraphics[trim=0 0 0 0,clip,width=0.45\linewidth]{figures/cs/0079_bev.jpg}
} \\

\vspace*{-2mm}
\caption{
\textbf{Qualitative results of DD3D applied on the Cityscapes3D~\cite{gahlert2020cityscapes} \emph{val}}. Cityscapes 3D contains bounding boxes of 6 types of vehicles (no pedestrian). In the bird-eye-view visualization (\textbf{left}), the concentric circles are $5$m apart. 
}
\label{fig:supp_results_qualitative_cs}
\end{figure*}

==> sections/qualitative_nusc.tex <==
\begin{figure*}
\vspace{-2mm}
\centering
% [trim=left bottom right top, clip]

\subfloat{
\includegraphics[width=0.49\linewidth]{figures/nusc/0076.jpg}
\includegraphics[trim=0 0 120 0,clip,width=0.38\linewidth]{figures/nusc/0076_bev.jpg}
} \\ 
\subfloat{
\includegraphics[width=0.49\linewidth]{figures/nusc/0035.jpg}
\includegraphics[trim=0 0 120 0,clip,width=0.38\linewidth]{figures/nusc/0035_bev.jpg}
} 
\vspace*{-2mm}
\caption{
\textbf{Qualitative results of DD3D applied on the nuScenes~\cite{caesar2020nuscenes} \emph{val}}. nuScenes contains bounding boxes of 10 object categories, including "Pedestrian", "Barrier" and "Traffic Cone", and "Construction Vehicle" (all shown above). We only show the results from front camera. 
}
\label{fig:supp_results_qualitative_nusc}
\end{figure*}

==> sections/rel_work.tex <==

% Current monocular 3D object detection algorithms can be categorized based on whether depth maps are inferred as an intermediate step or representation: RGB-only detectors and Depth-based detectors.
We review related 3D object detection methods as part of two main paradigms, depending on how whether depth is handled explicitly (i.e. via lifting or as an intermediate representation) or not. Additionally, we include a section reviewing the task of monocular depth estimation itself.
\\
% \noindent\textbf{RGB-only 3D detectors.}
\subsection{RGB-only 3D detectors}
As one of the early methods, Mono3D~\cite{chen2016monocular}, provides promising results in this direction using different semantic and shape cues to score a set of over-sampled 3D proposals. While only an RGB image is required at test time, scene constraints and additional priors are needed during training.
OFTNet~\cite{roddick2018orthographic} extends the idea of Mono3D and conduct joint proposal inferences on orthographic birds-eye-view without an explicit notion of depth.
Later RGB-only 3D detectors are normally built on top of a 2D object detector and further extract 3D object information exploiting 3D geometry priors and 3D-2D consistency~\cite{mousavian20173d,kehl2017ssd,ku2019monocular}. 
Mousavian et al.~\cite{mousavian20173d} explore the representations for direct 3D bounding box regression as well as losses that connect bounding box level 3D-2D projection error.~\cite{chen2020monopair} propose to encode pairwise spatial relationships
for partially-occluded objects from their adjacent neighbors, leading to improved detection results, while~\cite{liu2021ground,cai2020monocular} use scene or object surfaces to impose additional constraints during the learning process. SSD-6D~\cite{kehl2017ssd}  replaces part of the regression task with a classification task and exploits contour consistency between 3D and 2D projection trained on CAD models. 
% Moving beyond 2D project losses, RoI-10D~\cite{manhardt2019roi} proposes to lift 2D proposals into 3D through a differentiable listing process and directly regress 3D boxes with respect to 3D ground truth.
M3D-RPN~\cite{brazil2019m3d} jointly generates 3D and 2D proposals with shared anchors yielding improved 3D detection results. MonoDIS~\cite{simonelli2019disentangling, simonelli2020disentangling} and Kinematic3D~\cite{brazil2020kinematic} tackle the increase in parametric complexity and number of losses and propose simplifying the training dynamic 
%and balancing the regression targets
through loss decomposition and uncertainty estimation.

% With the increased complexity in parameterization and losses of these works, MonoDIS~\cite{simonelli2019disentangling, simonelli2020disentangling} and Kinematic 3D~\cite{brazil2020kinematic} look into simplifying the training dynamic and balance the regressions through loss decomposing and uncertainty estimation. 
%
More recent works also explore even more fine-grained regression of 3D objects embracing the recent advances in techniques like differentiable rendering~\cite{beker2020monocular} or 3D key-point detection~\cite{ barabanau2019monocular}. Recent approaches based on dense keypoint regression also estimate 3D bounding box locations of objects in the scene~\cite{barabanau2019monocular,liu2020smoke,zhou2019objects}.  Instead of sparse semantic supervision, our focus is on using raw unlabeled data as a proxy task via dense depth supervision during the pre-training stage. Unlike~\cite{liu2020smoke} our network architecture leverages hierarchical predictions which are aggregated across different FPN levels; additionally, we use a different box parameterization, and also output a 3D confidence which has been shown to improve overall detection accuracy~\cite{simonelli2019disentangling}.

% However, most the of the existent methods reply on complicated multi-network or multi-stage framework making it non-trivial to leverage additional data without 3D annotations (e.g. Image-Lidar pairs). 
% SMOKE~\cite{liu2020smoke} is recently proposed as the first end-to-end single-stage 3D detection directly regress 3D proposal and 3D keypoints. 

% \noindent\textbf{Depth-based 3D detectors.}
\subsection{Depth-based 3D detectors}
% \jie{Not sure if we should mentioned stereo-based method here as they are not monocular detectors.}
The other category of works generate depth maps from RGB images as an intermediate task. 
The generated depth can be used as an additional modality or dimension to provide additional constraints~\cite{manhardt2019roi,xu2018multi}.
ROI-10D~\cite{manhardt2019roi} employ an additional loss on the position of 3D bounding boxes using depth predicted by~\cite{pillai2019superdepth}.
Xu et al.~\cite{xu2018multi} adapt depth maps as additional feature layers at multiple stage of a detection network.
%
Another intuitive usage of the generated depth maps is converting RGB images into 3D point clouds (Pseudo-Lidar)~\cite{weng2019monocular, qian2020end, wang2020train,ma2019accurate}. The converted point clouds can be used in different Lidar-based 3D object detectors~\cite{wang2020train, qian2020end}.~\cite{wang2020train} combines 2D object bounding boxes and depth map to build a point cloud frustum~\cite{qi2018frustum} for each proposal which is then fed into a Lidar-based detector.~\cite{vianney2019refinedmpl} leverage sparsification and achieve state-of-the-art results with as little as $5\%$ of the original  points.~\cite{qian2020end} proposed to join the depth network and detector network jointly through a novel change of representation (COR) layer for information propagation. PatchNet~\cite{ma2020rethinking} also uses 2D proposal boxes combined with depth estimation and challenges the Pseudo-Lidar (PL) representation as the optimal way to use depth in 3D detection, yet a high quality depth map remains a key component in the algorithm. While PL-based detectors have shown great performance, some limitations remain: while implied, the relationship between depth quality and detection accuracy is not yet known. Moreover, recent work~\cite{simonelli2020demystifying} has exposed an underlying bias in the way PL monocular detectors are trained, casting doubt on some of the latest results as well as their ability to generalize.


% The Pseudo-Lidar or Depth-map based method presents promising results that indicate the important role of depth estimation in 3D object detection. 
% However, fewer works have been done looking into the correlation between the quality and property of the depth network and the resulting 3D object detection.
% Recently, Simonelli et al.~\cite{simonelli2020demystifying} express concerns over over-fitting and information-leak problem in these depth-based detectors considering the additional data used in the depth models. 
% In this work, we take a closer look at how we can improve the quality of depth network for 3D object detection without information leak. 
% \todo{yet to include the followings.}
%~\cite{cai2020monocular},  


\subsection{Monocular Depth Estimation}

Estimating depth from a single image is inherently an ill-posed problem, since an infinite number of 3D scenes can correspond to the same 2D plane. Even so, it has recently been shown~\cite{eigen2014depth} that a neural network can be trained to produce per-pixel depth estimates from single images, by learning appearance-based features from a set of labeled images. 
Since then, a substantial amount of work has been done to improve the accuracy and performance of supervised monocular depth estimation~\cite{depthcrf,huberloss,packnet-semisup,normalscvpr2,selfsupsem,packnet-semguided,fouriercvpr,dorncvpr,lee2019big}, as well as its extension to the self-supervised domain~\cite{pillai2018superdepth, zhou2018stereo, ummenhofer2017demon,packnet,godard2018digging2,vijayanarasimhan2017sfm}. While self-supervision enables training with unlabeled images (stereo pairs or videos), it is important to note that the generation of depth labels for supervised training does not require human annotation, which is the case for tasks such as 3D object detection. It only requires an additional sensor (e.g., LiDAR) during data collection, which enables the efficient generation of large-scale datasets, such as the one used in this work. 


%%%%%%%%%%META NOTES
% qi2018frustum

% vianney2019refinedmpl

% weng2019monocular: Monocular 3D Object Detection with Pseudo-LiDAR Point Cloud
% 2D proposal + Pseudo-lidar  --> point frustum --> 3D segmentation / regression , multi stage, 3D-2D consistency loss

%qian2020end: End-to-End Pseudo-LiDAR for Image-Based 3D Object Detection
% Jointly train depth network and a Psudo Lidar 3D det network, COR; change of represenation layer

%wang2020train: Train in Germany, Test in The USA: Making 3D Object Detectors Generalize
% first domain adaptation analysis in 3D Det.
% Solutions: Fewshot finetuning / statistic normalization. 

% you2019pseudo: PseudoLidar ++
% Improved stereo based depth network: disparity volumn --> depth volumn (SDN)
% further improve using 4-beam lidar through depth-propagetion inspired by graph-based manifold learning.

%% 
% chen2020monopair: Monocular  3d  object  detection  using  pairwisespatial relationships
% encode spatial constraints for partially-occluded objects from their adjacent neighbors. uncertainty aware predictions for object locations and 3D distances forthe adjacent object.pairs,



% cai2020monocular

% ma2020rethinking
%philion2020lift
% hahner2020quantifying

%simonelli2020demystifying



==> sections/results.tex <==
% We present detailed analysis on our pretraining and finetuning strategy, as well as benchmark results of our two proposed detectors on three 3D detection benchmarks.
\subsection{3D detection}
\label{subsec:3d_detection}

\input{sections/results_3D_det}

\subsection{The impact of data on depth and 3D detection}
\label{subsec:depth_pretraining}

% \begin{figure}[h]
%     \includegraphics[width=0.99\columnwidth,trim={0mm 0mm 0mm 0mm},clip]{figures/scaling_law.pdf}
%     \caption{Accuracy of 3D detection continues to improve, at least up to 1.89M images used for pre-training. We pre-train FCOS-3D with growing sizes of image-pointcloud pairs until convergence. The models are then fine-tuned on for 3D detection on KITTI \emph{train}, and evaluated on KITTI \emph{val}.}
%     \label{fig:pretraining_vs_depth}
% \end{figure}


\begin{figure}[t!]
    \includegraphics[width=0.99\columnwidth,trim={0mm 0mm 0mm 0mm},clip]{figures/scaling_laws/fcos_and_PL.png}
    \caption{\textbf{DD3D and PL are pre-trained with varying dataset sizes} and fine-tuned for 3D detection on the KITTI3D training split, and evaluated on the KITTI3D validation split. As shown, the accuracy of both 3D detectors continues to improve, at least up to the 2.5M images (25K split) used for pre-training.}
    \label{fig:pretraining_vs_depth}
\end{figure}

\begin{figure}[h]
    \includegraphics[width=0.99\columnwidth,trim={0mm 0mm 0mm 0mm},clip]{figures/scaling_laws/depth_vs_3d_det.png}
    \caption{\textbf{We evaluate depth performance (abs\_rel) against PL 3D detection performance (Car 3DAP$|_{R_{40}}$) at each pre-training step.} Our results indicate an almost perfect linear relationship between depth quality and 3D detection accuracy. All results are computed on the KITTI3D validation split.}
    \label{fig:3d_vs_depth}
\end{figure}

We explore the interplay between data, 3D detection, with our results summarized in Fig.~\ref{fig:pretraining_vs_depth}. The complete results are presented in the supplementary. We note that both approaches benefit from increased amounts of unlabelled data. As mentioned in Sec.~\ref{subsec:3d_detection}, we record better performance for the PL detector compared to DD3D on the KITTI3D val set which, however, does not seem to transfer to the test set.  

Additionally, we evaluate depth quality against the 3D detection accuracy of the PL detector, with results shown in Fig.~\ref{fig:3d_vs_depth}. Our results indicate an almost perfect linear relationship between depth quality as measured by the \textit{abs\_rel} metric and 3D detection accuracy for our PL-based detector.

% we expect a monotonic increase in PL 3D detection accuracy with data, the exact relationship


% As expected, depth quality as measured by the \emph{abs\_rel} metric improves with additional data (Fig~\ref{fig:scaling_laws_packnet} left). Note that our monocular depth estimator $PackNet$~\cite{packnet} is trained completely from scratch, without any ImageNet~\cite{deng2009imagenet} pretraining. Conversely, we note a direct correlation between the depth quality and 3D detection (Fig~\ref{fig:scaling_laws_packnet} middle). We summarize the relationship between depth and 3D detection in (Fig~\ref{fig:scaling_laws_packnet} right, noting an almost linear relationship between the \textit{abs\_rel} depth metric and 3D detection. 

% \begin{figure*}[t!]
% % \vspace{-1mm}
% \centering

% \subfloat{
% \includegraphics[width=0.3\linewidth]{figures/scaling_laws/PacknetFT_depth_metrics_k3d_val_abs_rel.png}
% \includegraphics[width=0.3\linewidth]{figures/scaling_laws/Packnet_3d_det.png}
% \includegraphics[width=0.3\linewidth]{figures/scaling_laws/depth_vs_3d_det_AP_3d_metrics_Mod.png}
% }
% \caption{
% \textbf{Depth quality vs 3D AP for varying dataset sizes.} \textbf{Left:} we report the \textit{abs\_rel} depth metric on the KITTI3D validation split; the depth network is pretrained with varying dataset sizes and fine-tuned on the KITTI Eigen-clean split. \textbf{Middle:} for each depth network, a PL 3D detector is trained on KITTI 3D train and evaluated on KITTI 3D val. \textbf{Right:} we plot the proposed abs\_rel metric vs the resulting 3D AP metric; note that both are computed on the KITTI 3D validation split.
% }
% \label{fig:scaling_laws_packnet}
% \end{figure*}

\input{tables/depth_vs_det2d}



\subsection{Ablative analysis}
\label{subsec:ablative}



\noindent\textbf{Depth vs. 2D detection.} To better quantify the effect of monocular depth pre-training applied on FCOS-3D, we attempt to isolate the role of pre-training methods through controlled experiments. Starting from a single set of initial parameters trained on MS-COCO dataset for 2D detection, we perform additional pre-training using a common set of images that are annotated with both 2D bounding box labels and sparse depth values obtained by projecting Lidar point-cloud.
The dataset used for pre-training is composed of 136571 images from nuScenes dataset~\cite{caesar2020nuscenes} \emph{train} set, after removing images that contains no bounding boxes. To further ensure the comparison is fair, we run the same number of training steps and batch size ($15000$ and $512$) with no data augmentation. The learning rate for each pre-training was chosen by validating on \emph{val} set ($0.01$ and $0.005$). To address variance from random initialization, we report the average of four runs for each setting.
The experiment shows that supervised monocular depth prediction consistently improves the the 3D detection accuracy for all categories \ref{table:pretraining_depth_vs_detection}.

%\noindent\textbf{Depth vs. 2D detection pre-training.} To better isolate and quantify the effect of monocular depth pre-training on the performance of FCOS-3D, we compare with other pre-training tasks in the same domain (i.e. autonomous driving). Specifically, using the nuScenes dataset~\cite{caesar2020nuscenes}, we perform experiments pre-training on either 2D detection or depth estimation, using the \emph{same} set of images, starting from a baseline model which is pre-trained on COCO~\cite{lin2014microsoft} for 2D detection. Our results are summarized in Table~\ref{table:pretraining_depth_vs_detection} (full results in supplementary), where \textit{2D-det} denotes 2D bounding box detection as the pre-training task, while \textit{Depth} denotes supervised depth prediction using ground-truth depth as pre-training. Following pre-training, all models are fine-tuned on the KITTI3D~\cite{geiger2012we} training split for 3D detection, with the metrics computed on the KITTI3D validation split. Our results indicate that depth pre-training is a superior task, significantly improving the baseline performance and surpassing other pre-training strategies. 

% We aim to ablate the role of pre-training on depth estimation with our results . 

% We use FCOS-3D to pre-train subset of parameters relevant to each pre-train task, and fine-tine on KITTI \emph{train} for 3D detection. \textbf{2D-det} denotes 2D bounding box detection as pre-training task; \textbf{Depth} denotes supervised depth prediction using ground-truth depth available from Lidar point-cloud. Starting from parameters pre-trained on MS-COCO dataset (2D detection), we perform additional pre-training in target domain (i.e. autonomous driving) on either 2D detection or depth estimation, using the \emph{same} set of images (\textbf{nusc}) until convergence. To understand how the accuracy scales with respect to the size of pre-train data, we internally collect a large set of image-Lidar pairs (\textbf{internal}) and use it for depth pre-training. The fine-tuned models are evaluated on KITTI \emph{val}. We only report "Moderate" metrics. Depth pretraining significantly improves 3D detection accuracy, up to \textbf{30.6\%} from the baseline pre-training method.


\input{tables/v2_99}

\input{sections/results_qualitative}

\noindent\textbf{Backbone analysis.} We perform an additional analysis on backbone type for FCOS-3D, showing result with the V2-99~\cite{lee2019centermask} and DLA-34~\cite{yu2018deep} architectures. For both networks we show the baseline results, as well as results after using monocular depth pre-training on the \textit{25K split} (2.5M images). All models are further fine-tuned for 3D detection on KITTI3D~\cite{geiger2012we} train, with numbers reported on KITTI3D val. We run each fine-tuning experiment four times, and report the average in Table~\ref{table:v2-99}. For both architectures we note an increase in performance following monocular depth pre-training. Interestingly, the larger backbone (V2-99~\cite{lee2019centermask} - 96.9M parameters) achieves very poor results without the proposed depth pre-training step; our results indicate that depth pre-training is key in obtaining good 3D detection performance for larger backbones, with significant performance jumps on the rare classes.

\input{tables/fcos_multitask}

\noindent\textbf{Multi-task fine-tuning.} All our 3D detection results up to this point have been obtained after fine-tuning FCOS-3D only on the downstream task of 3D detection. We regard this as an advantage of our approach compared to PL-style detectors that require specialized fine-tuning of the depth component in the target domain. As an additional experiment, we investigate the performance of FCOS-3D when fine-tuning both the depth and 3D detection in the target domain, i.e. in a multi-task setting. Our findings are summarized in Table~\ref{table:fcos_multitask}, with full details in the supplementary. We note a slight performance increase on car performance and pedestrian performance as well as a performance decrease for cyclists. These preliminary results indicate that depth fine-tuning has marginal benefits when combined with 3D detection in a multi-task framework. 



% Pre-training on supervised depth estimation allows for training larger backbone of FCOS-3D, as shown in Table.~\ref{table:v2-99}. We pre-train V2-99 \cite{lee2019centermask} backbone (96.9M parameters) using 2D detection on MS-COCO dataset, and perform additional pre-training using depth prediction on our internal dataset of image-pointcloud pairs. The models are then fine-tuned on KITTI \emph{train} for 3D detection, and evaluated on KITTI \emph{val}. The depth pre-training significantly improve rare classes: 4$\times$ for "Pedestrian", 37$\times$ for "Cyclist". We run each fine-tuning experiment four times, and report the average. We only report "Moderate" metrics due to limited space.

\subsection{Qualitative results}
\label{subsec:qualitative}


We show qualitative results in Figure~\ref{fig:results_qualitative}, with the right hand-size showing a top-down birds-eye-view projection of the predicted (red)boxes. Our method is capable of accurately detecting objects in different poses, orientations, and at different ranges, including under heavy occlusions.

==> sections/results_3D_det.tex <==
% \input{tables/kitti3d_test_multi_2}

\input{tables/kitti3d_val}

\noindent\textbf{KITTI-3D} We show in Table~\ref{table:kitti_3d_val} the effect of pre-training (sub-)networks of the two types of 3D detectors, PL and DD3D using a large scale dataset of images and Lidar frames. We use \emph{2.5M-set} for depth pre-training, and report 3D Box AP$|_{R_{40}}$ metric on \emph{val} set of KITTI-3D.

The baseline models for DD3D are initialized by FCOS models trained to predict 2D bounding box on COCO dataset, which yields $40.14\%$ and $44.1\%$ \emph{mAP} on COCO \emph{val} set. The models are then fine-tuned to predict 3D bounding box using \emph{train} set of KITTI-3D. The depth-pretrained counterparts (\emph{Depth pre-trained}) are instead pre-trained to predict dense depth using the 2.5M-set, followed by the same fine-tuning on \emph{train} of KITTI-3D. We report comparisons for two backbones, DLA-34~\cite{yu2018deep} and V2-99~\cite{lee2019centermask}.%, and use 3D Box AP$|_{R_{40}}$ metric.

Replacing the 2D detection pretraining (COCO) with the depth pretraining (2.5M-set) yields significant improvement in 3D detection accuracy, i.e. $\textbf{2.51\%} \sim \textbf{4.89\%}$ APs for DLA-34 backbone.  We also note the depth pre-training itself can be initialized by the COCO pre-trained models. For DLA-34 backbone, this yields $1.79\% \sim 2.24\%$ additional improvements, when compared pre-training with 2.5M-set from scratch. Lastly, we observe that depth pre-training is more effective in pre-training backbones with large capacity, e.g. V2-99, yielding $\textbf{7.27\%} \sim \textbf{11.45\%}$ gain in APs.

The baseline model for PL uses a depth network trained on eigen-clean set of KITTI-Depth dataset to estimate dense depth map of each image in \emph{train} of KITTI-3D. We then follow the same PL pipeline proposed by \cite{qi2018frustum, ma2020rethinking} to predict 3D bounding from the RGB-D images. The depth-pretrained counterpart of PL approach is identical to the baseline model, but is preceded by additional stage of training depth network using the 2.5M-set. We observed that for PL, pre-training the depth network in the target domain (i.e. eigen-clean) \emph{after} the large-scale out-of-domain pre-training (i.e. 2.5M-set) is important, because the output depth values are directly used as depth estimate of 3D bounding boxes.  

The table shows that large-scale depth pre-training also significantly improve the accuracy for PL, i.e. $\textbf{8.56\%} \sim \textbf{16.90\%}$ gain in APs. Overall, the improvements from the depth pre-training, both DD3D and PL, are clearly larger than the gain that other methods that have reported on \emph{val} set of KITTI-3D.

%\noindent\textbf{KITTI3D} Our numbers on the \textit{validation split} of the KITTI3D dataset are summarized in Table~\ref{table:kitti_3d_val} for the BEV and 3D detection tasks. We note that our baseline numbers are on par with related methods, and we record a significant increase in performance when using the modifications proposed in this paper. Our baseline FCOS-3D model uses COCO~\cite{lin2014microsoft} pre-training and we record an increase of $22\%$ by using depth estimation as an auxiliary task for pre-training ($17.03$ vs $13.96$). Our PL numbers improve over the current state-of-the-art on this split by $59\%$ and over our baseline by $76\%$ ($22.36$ vs $14.10$ and $12.70$ respectively). Note that we are omitting from this comparison the results reported by methods that use depth trained on images that overlap with the KITTI3D train and val splits. 

%\input{tables/kitti3d_test}
% New results: 16.34% BoxAP, , Car, Moderate
\input{tables/kitti3d_test}

Similar conclusions also hold on official KITTI-3D benchmark (Table~\ref{table:kitti_3d_test}).  We report the results of PL and DD3D pre-trained by 2.5M-set and fine-tuned on the combined set of \emph{train} and \emph{val} sets of KITTI-3D. Our PL model, when using the improved depth estimator, outperforms most of the the existing PL methods, and perform competitively with \cite{simonelli2020demystifying} which uses 3D uncertainty to modulate the confidence. The DD3D model outperforms all existing monocular methods in all \emph{Car} metrics, with significant difference from the second-best approaches ($\textbf{3.16\%}$ $\sim$ $\textbf{4.15\%}$). Notably, DD3D features simple single-stage architecture and makes no use of explicit temporal or geometric cues.

% This is here due to formatting issues
\input{tables/kitti3d_test_multi_2}


%This further highlights the difficulties of properly training a PL detector, while ensuring that no statistical leakage exists between the depth estimation and the 3D detection splits. Our findings are in line with those of~\cite{simonelli2020demystifying}, i.e. an unbiased depth split (Eigen clean vs Eigen train) still seems to lead to overfitting on the KITTI3D val set and poor generalization to the KITTI3D test set. Conversely, \textit{FCOS-3D} requires no additional fine-tuning other than the downstream task (i.e. 3D detection) on the target domain, simplifying deployment greatly. 

%Our numbers on the \textit{test split} of the KITTI3D dataset are reported in Table~\ref{table:kitti_3d_test}. Our novel single-stage 3D detector (\txtit{FCOS-3D}) outperforms all other single and two-stage detectors, with a notable improvement of up to $21\%$ over the previous best published results (i.e. Car - Easy category 3DAP $20.09$ vs. $15.54$). Our PL-based detector also outperforms the previous state-of-the-art for the BeV metric, achieving competitive results with~\cite{simonelli2020demystifying}. Interestingly, our PL detector achieves better results on the KITTI3D validation split compared to FCOS-3D, however, FCOS-3D performs much better on the test set. This further highlights the difficulties of properly training a PL detector, while ensuring that no statistical leakage exists between the depth estimation and the 3D detection splits. Our findings are in line with those of~\cite{simonelli2020demystifying}, i.e. an unbiased depth split (Eigen clean vs Eigen train) still seems to lead to overfitting on the KITTI3D val set and poor generalization to the KITTI3D test set. Conversely, \textit{FCOS-3D} requires no additional fine-tuning other than the downstream task (i.e. 3D detection) on the target domain, simplifying deployment greatly. 

We also report KITTI3D test split results on \textit{Pedestrians} and \textit{Cyclists} in Table~\ref{table:kitti_3d_test_multi_class}, noting a $\mathbf{59.7\%}$ increase in AP on \textit{Pedestrians} compared to the best published result to date on this dataset (i.e. $9.28$ vs $5.81$). We also outperform all methods on \textit{Cyclists} except for~\cite{chen2020monopair}, which however performs worse than DD3D in other two classes. 

 

% in this category by a significant margin - for Car - medium our 3DAP is $11\%$ higher (i.e. $13.05$ vs $11.72$). 

% ; our improvements are significantly more noticeable on smaller classes (i.e. cyclists and pedestrians), as reported in the supplementary

\noindent\textbf{nuScenes.} To further validate our contributions, we report results on the nuScenes~\cite{caesar2020nuscenes} dataset official test set. To generate our test submissions, we use test-time augmentation by resizing test images by factors between 70\% and 130\%. Our results on the nuScenes dataset are presented in Table~\ref{table:nuscenes_test_summary}, where we report summary detection metrics averaged over all $10$ categories of the \emph{nuScenes Detection Challenge}. We note that our method outperforms the best previously published 3D monocular detection~\cite{simonelli2020disentangling}, with our \textit{mAP} metric even surpassing the PointPillars~\cite{lang2019pointpillars} lidar based detector. In Table~\ref{table:nuscenes_test_detailed} we show detailed \textit{Average Precision} metrics for all distance thresholds for the \textit{Car}, \textit{Pedestrian} and \textit{Cyclist} categories. Our method outperforms all published baselines on 11 out of 12 metrics. As with our results on the KITTI3D dataset, we note that our method almost doubles the best published number to date on \textit{Pedestrians} on the strictest threshold (i.e. AP at 0.5m 12.5 vs 6.7); we record a similar performance gain on the \textit{Car} category (i.e. 19.6 vs 10.6).

% Due to the limited space, we report the \textit{Average Precision} for each class and the mean \emph{AP}, and report detailed results on the \textit{Car}, \textit{Pedestrian} and \textit{Bicycle} classes in the supplementary. 

\input{tables/nuscenes_summary}

\input{tables/nuscenes_results}



% \noindent\textbf{CityScapes3D.} Our results are summarized in Table~\ref{table:cityscapes_test_results}, where we report per class \textit{Detection Score (DS)} results as well as the \textit{AP}, \textit{BEV} and \textit{OS Yaw} summary metrics.

% \input{tables/cityscapes_results}

==> sections/results_qualitative.tex <==
\begin{figure*}[t!]
\vspace{-2mm}
\centering
% [trim=left bottom right top, clip]
% \subfloat{
% \includegraphics[width=0.55\linewidth]{figures/qualitative_new/000020.jpg}
% \includegraphics[width=0.21\linewidth]{figures/qualitative_new/000020_bev.jpg}
% } \\ 
\subfloat{
\includegraphics[width=0.55\linewidth,height=3cm]{figures/qualitative_new/000022.jpg}
\includegraphics[width=0.21\linewidth,height=3cm]{figures/qualitative_new/000022_bev.jpg}
} \\ 
\vspace*{-2mm}
\subfloat{
\includegraphics[width=0.55\linewidth,height=3cm]{figures/qualitative_new/000023.jpg}
\includegraphics[width=0.21\linewidth,height=3cm]{figures/qualitative_new/000023_bev.jpg}
} \\ 
% \subfloat{
% \includegraphics[width=0.55\linewidth]{figures/qualitative_new/000075.jpg}
% \includegraphics[width=0.21\linewidth]{figures/qualitative_new/000075_bev.jpg}
% } \\
% \subfloat{
% \includegraphics[width=0.55\linewidth]{figures/qualitative_new/000247.jpg}
% \includegraphics[width=0.21\linewidth]{figures/qualitative_new/000247_bev.jpg}
% } \\ 
% \subfloat{
% \includegraphics[width=0.55\linewidth]{figures/qualitative_new/000454.jpg}
% \includegraphics[width=0.21\linewidth]{figures/qualitative_new/000454_bev.jpg}
% } 
\vspace*{-2mm}
\caption{
\textbf{Qualitative detections obtained by the proposed FCOS-3D architecture.} Left: 3D box projection into the image. Right: Top-down birds-eye-view visualization of the predicted boxes. Results generated on images from the KITTI3D~\cite{geiger2012we} test set. We show additional results on CityScapes3D~\cite{gahlert2020cityscapes} and nuScenes~\cite{caesar2020nuscenes} in the supplementary.
}
\label{fig:results_qualitative}
\end{figure*}

==> suppmat.tex <==
\section{Introduction}
The goal of this supplementary document is to provide additional details complementing our main paper: detailed Pseudo-Lidar results - Section~\ref{sec:pretraining_detailed}; detailed nuScenes~\cite{caesar2020nuscenes} results - Section~\ref{sec:nusc_detailed}; Cityscapes3D~\cite{gahlert2020cityscapes} results - Section~\ref{sec:cityscapes}; detailed DD3D fine-tuning results - Section~\ref{sec:fcos_ablative}; depth pre-training schedule - Section~\ref{sec:pretraining}; Pseudo-Lidar 3D confidence head implementation details - Section~\ref{sec:pl_detection_head}; DD3D architecture details - Section~\ref{sec:fcos_architecture}; qualitative results - Section~\ref{sec:qualitative}.


% on (i) the experimental results presented in the main paper that were omitted due to lack of space and (ii) the architectures and training setup of the FCOS-3D and Pseudo-Lidar approaches to facilitate the reproduction of our results.

\section{Pseudo-Lidar detailed results}
\label{sec:pretraining_detailed}

% We pre-train our monocular depth estimator PackNet~\cite{guizilini20203d} on 4 splits (\textit{1K}, \textit{5K}, \textit{10K}, \textit{25K}), as well as starting from scratch. Following this pre-training stage, we fine-tune the depth estimator on the KITTI3D~\cite{geiger2012we} \textit{Eigen clean} depth split. Finally, for each depth model we train a Pseudo-Lidar 3D detector using the KITTI3D train split.
In this section we present detailed depth and 3D detection results, complementing the summary presented in Fig. 4 in the main submission. These results are summarized in Table~\ref{table:supp_pl_data_vs_det}, where we note the trend of improving with data for both the depth and the 3D detection results, as well as the correlation between the two. 

\input{tables/pl_data_vs_det}

\section{nuScenes~\cite{caesar2020nuscenes} detailed results}
\label{sec:nusc_detailed}
\input{tables/nuscenes_per_class}

We present detailed results for all the object categories in Table~\ref{table:supp_nuscenes_per_class} (note that this complements Table 5 from the main paper). In addition, we present per-category metrics in terms of the three true-positive metrics used in nuScenes, i.e., Average Precision (AP), Average Translation Error (ATE), Average Scale Error (ASE) and Average Orientation Error (AOE) in Table~\ref{table:supp_nuscenes_all} (note that this complements the summary metrics presented in Table 4 of the main submission). We compare against the previous monocular state-of-the-art, MonoDis~\cite{simonelli2020disentangling}, and a widely used Lidar-based method, PointPillars~\cite{lang2019pointpillars}, in Table~\ref{table:supp_nuscenes_all}. We consistently outperform MonoDis  across most metrics, and even outperform PointPillars on average. Our method is particularly robust in detecting the long-tail of objects in rare categories.

\input{tables/nuscenes_all}

% We present additional ablative experiments on pre-training using supervised depth prediction on the CityScapes3D dataset~\cite{gahlert2020cityscapes}. As done in Sec 5.2 of the main text, we measure the effect of performing additional pre-training using the "25K split" of the internal dataset, cf. Fig.3 of the main text. The only differences between the experiments on KITTI3D are that (i) we used class balanced sampling~\cite{Gupta_2019_CVPR} to address the imbalance between categories, and (ii) we used a new set of hyper-parameters in training ($0.008$ for learning rate, $32$ for batch size, $30000$ for training steps). We use the DLA-34\cite{yu2018deep}  backbone, and train the models on the \emph{train} subset, and evaluate on the \emph{val} subset of Cityscapes3D~\cite{gahlert2020cityscapes}. We report the average of $4$ models initialized with different random seeds during training.

\section{Cityscapes3D~\cite{gahlert2020cityscapes} results}
\label{sec:cityscapes}
In addition to KITTI3D~\cite{geiger2012we} and nuScenes~\cite{caesar2020nuscenes}, we also evaluate our method on the Cityscapes3D~\cite{gahlert2020cityscapes} benchmark. This novel dataset provides 3D object annotations using stereo depth, and thus provides an interesting alternative to other 3D datasets where objects are annotated in the lidar point cloud and then projected into the camera images. As done in Sec 5.2 of the main text  (cf. Fig.3 of the main submission), we measure the effect of performing additional pre-training using the "25K split" of the internal dataset. The only differences with the experiments on KITTI3D are that (i) we used class balanced sampling~\cite{Gupta_2019_CVPR} to address the imbalance between categories, and (ii) we used a new set of hyper-parameters in training ($0.008$ for learning rate, $32$ for batch size, $30000$ for training steps). We use the DLA-34\cite{yu2018deep}  backbone, and train the models on the \emph{train} subset, and evaluate on the \emph{val} subset of Cityscapes3D~\cite{gahlert2020cityscapes}. We report the average of $4$ models initialized with different random seeds during training. 

Our results are summarized in Table~\ref{table:supp_cityscapes_val_results}, where we report the same metrics used by nuScenes dataset in Table~\ref{table:supp_nuscenes_per_class}, i.e.,  average precision per class as well as the \emph{mean AP}. To the best of our knowledge, we are the first to evaluate metrics on this dataset, as no vision-only baselines exist. We argue that (i) the large gap in detection accuracy between nuScenes and CityScapes3D is mainly due to the difference in the size of training data ($\sim$1M vs. $\sim$3K), and (ii) the gap is significantly overcome by using parameters pre-trained on depth prediction ($14.38\%$ vs. $22.55\%$). 

% we compute and report in Table~\ref{table:supp_cityscapes_val_results} the Average Precision following the nuScenes~\cite{caesar2020nuscenes} format (i.e. we compute the AP over 4 distance thresholds, reporting the average), and note similar performance across the nuScenes and Cityscapes3D datasets. We also report the baseline performance in Table~\ref{table:supp_cityscapes_val_results}, noting as before a significant increase in performance when pre-training FCOS-3D with monocular depth estimation. 

% \input{tables/cityscapes_results}
\input{tables/cs_nusc}


%\section{FCOS-3D ablative analysis (fine-tuning): detailed results}
\section{Fine-tuning DD3D with RoI-focused depth supervision}
\label{sec:fcos_ablative}

\input{tables/results_multi_task}
In Table 8 of the main submission, we present an abridged version of the full KITTI benchmark results showing the effect of using auxiliary depth loss computed on region-of-interest (RoI), while fine-tuning DD3D for 3D detection. In Table~\ref{table:supp_detailed_multi_task}, we present the full benchmark results that include "Easy" and "Hard" metrics for all object categories. The conclusion remains unchanged: additional depth fine-tuning on the target domain marginally improves performance on some classes, while decreasing performance on others. That is, fine-tuning depth prediction on target domain yields only marginal gain over the pre-training using large-scale image-Lidar data. Note that this is in contrast to Pseudo-Lidar methods, which require a specialized fine-tuning step for the detection networks in the target domain.

% To recapitulate, we explored the potential of using Lidar point-cloud in the target domain (in this case KITTI scenes) by adding a loss measuring the mean L1-distance of predicted and ground-truth depth to the 3D detection losses of FCOS-3D. 
%We present detailed 3D detection results in Table~\ref{table:supp_detailed_multi_task} (note that these results complement the results presented in Table 8 of the main submission). The numbers indicate that additional depth fine-tuning on the target domain marginally improves performance on some classes, while decreasing performance on others. Note that this is in contrast to Pseudo-Lidar methods, which require a specialized fine-tuning step for the detection networks in the target domain.

\section{Details of depth pre-training}
\label{sec:pretraining}
We provide the full details of the training schedule used for supervised monocular depth pre-training of both DD3D and PackNet.

\noindent\textbf{DD3D.} For all supervised depth pre-training splits (1K, 5K, 10K, 25K), we use L1 loss between predicted depth and projective ground-truth depth, and $256$ as batch size. The size of input images (and projected depth map) is 1600 $\times$ 900, and we resize them into 910 $\times$ 512. When resizing the depth maps, we perserved the sparse depth values by assigning all non-zero depth values to the nearest-neighbor pixel in the resized image space (Note that this is different from naive nearest-neighbor , where the target depth value is assigned zero, if the nearest-neighbor pixel in the original image does not have depth value.) We observed the training converges after 15 epochs. We use momentum optimizer with $\beta = 0.99$.  

\noindent\textbf{PackNet.} We train the monocular depth estimation network PackNet~\cite{guizilini20203d} on each pre-training split. In each case we use a batch size of $4$, constant learning rate of $5e^{-5}$, input resolution of $640\times 480$ and the Adam~\cite{loshchilov2017decoupled} optimizer with $\beta_1=0.9$ and $\beta_2=0.999$. We train until convergence on each split (1K, 5K, 10K, 25K), i.e. until the depth metrics computed (see Table~\ref{table:supp_pl_data_vs_det}) stabilize. Specifically, for each split we trained for 20 epochs, with the exception of 1K where we noticed convergence after 10 training epochs. 

% The training splits contain an increasing number of images, as follows: 1K: $10^6$ images, 5K: $5\cdot 10^6$ images, 10K: $10 \cdot 10^6$ images, 25K: $25 \cdot 10^6$ images. For each we train until convergence, i.e. until the depth metrics computed (see Table~\ref{table:supp_pl_data_vs_det}) stabilize. 

\section{Pseudo-Lidar 3D confidence head}
\label{sec:pl_detection_head}

Our PL 3D detector is based on~\cite{ma2020rethinking}, and outputs 3D bounding boxes with 3 heads, separated based on distance (i.e. near, medium and far). Following~\cite{simonelli2019disentangling,simonelli2020demystifying} we modify each head to output a 3D confidence, trained through the 3D bounding box loss as described in the main submission. Specifically, each 3D box estimation head consists of 3 fully connected layers with dimensions $512 \longrightarrow 512 \longrightarrow 256 \longrightarrow  \left(\delta,\gamma\right)$, where $\delta$ denotes the bounding box parameters as described in~\cite{ma2020rethinking}, and $\gamma$ denotes the 3D bounding box confidence.

\section{DD3D architecture details}
\label{sec:fcos_architecture}

\noindent\textbf{FPN} As described in \cite{lin2016fpn}, a feature pyramid network (FPN) is composed of \emph{bottom-up} network which is a feed-forward CNN that computes feature maps with a scaling step of 2, and a \emph{top-down} network with lateral connections that recovers high-resolution features from low-resolution ones. We use two types of bottom-up network, DLA-34 \cite{yu2018deep} and V2-99 \cite{lee2019centermask}. Both FPNs yield 5 levels of feature maps. For DLA-34, the FPN features are first computed across three levels (with step size of 8, 16, and 32) using the standard FPN computation \cite{lin2016fpn}, and then two lower resolution features (with step size of 64, 128) are computed by stacking two $3\times3$ 2D convolution with stride equals to 2 on top of highest level features of FPN (See Fig 2 of the main paper for an illustration). For V2-99, the bottom-up network (and therefore the standard FPN features) by default produces 4 levels of features (step size = 4, 8, 16, and 32). We create an additional level of features by adding one $3\times3$ 2D convolution. Note that the final resolution of FPN features derived from DLA-34 and V2-99 network is different, DLA-34 computes features with step sizes equal to 8, 16, 32, 64, and 128, while V2-99 computes the ones that are equal to 4, 8, 16, 32, and 64. 

\noindent\textbf{2D detection head} 
For 2D detector, we closely follow the decoder architecture and loss formulation of the original FCOS~\cite{tian2019fcos}.
In addition, we adopt the recent changes introduced in the updated version~\cite{fcos-arxiv} in positive sampling approach.
%The only difference from the original FCOS \cite{tian2019fcos} is the recently introduced matching strategy, i.e. how to match CNN features to each object (or its 2D bounding box).
Recently, the authors of~\cite{tian2019fcos} showed that center-based positive sampling, as suggested in~\cite{zhou2019objects}, yields additional gain in 2D detection accuracy.
%That is, instead of using all CNN features that falls within the 2D bounding box, one uses only the features that are close to the center of the bounding box. We adopt this matching strategy for matching. 
Under the new center-based approach, only the center-portion of the gound truth bounding box are used to assign positive samples in $\mathcal{L}_{reg}$ (Eq. 3); see~\cite{fcos-arxiv} for additional details.


\section{The impact of data on depth and 3D detection}
\label{sec:supp_data_vs_3d_det}

We evaluate depth quality against the 3D detection accuracy of the PL detector, with results shown in Fig.~\ref{fig:3d_vs_depth}. Our results indicate an almost perfect linear relationship between depth quality as measured by the \textit{abs\_rel} metric and 3D detection accuracy for our PL-based detector.

\begin{figure}[h]
    \includegraphics[width=0.99\columnwidth,trim={0mm 0mm 0mm 0mm},clip]{figures/scaling_laws/depth_vs_3d_det_v2.png}
    \caption{\textbf{We evaluate depth performance (abs\_rel) against PL 3D detection performance (Car 3DAP$|_{R_{40}}$) at each pre-training step.} Our results indicate an almost perfect linear relationship between depth quality and 3D detection accuracy. All results are computed on the KITTI3D validation split.}
    \label{fig:3d_vs_depth}
\end{figure}

\section{Qualitative results}
\label{sec:qualitative}

We present additional qualitative results on Cityscapes3D~\cite{gahlert2020cityscapes} in Figure~\ref{fig:supp_results_qualitative_cs}, KITTI~\cite{geiger2012we} in Figure~\ref{fig:supp_results_qualitative} and nuScenes~\cite{caesar2020nuscenes} in Figure~\ref{fig:supp_results_qualitative_nusc}. To generate the qualitative results we apply non-maxima suppression (NMS) with 0.3 as threshold on intersection-over-union (IoU). We show detected bounding boxes with confidence higher or equal to 0.4. We also refer readers to the supplementary video that shows the DD3D output on the nuScenes \emph{val} images, which are videos sampled at 2Hz, along with a high-level overview of our paper.
\input{sections/qualitative_cs}

\input{sections/qualitative}

\input{sections/qualitative_nusc}



==> tables/ablation_2d_mask_type.tex <==

\begin{table}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Depth net}& 
Easy & 
Med &
Hard &
Easy & Med & Hard \vspace{0.5mm}\\
\midrule
PackNet & 
41.59 & 
27.75 &
23.69 &
30.91 &
20.53 &
17.25
\\
PackNet + 2D masks  & 
40.46 & 
27.64 & 
23.03 &
32.39 &
21.29 & 
17.97 
\\

PackNet + Gauss. masks &
43.46 &
29.96 &
25.07 &
34.01 &
22.31 &
18.58 
\\



\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{Ablative analysis of 3D detection performance with different depth fine-tuning strategies.}}
\label{table:baseline_depth_detection}
}
\end{table}

==> tables/ablation_depth_detection.tex <==

\begin{table*}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
% \rowcolors{2}{lightgray}{white}
\begin{tabular}{llll|cccccc|cccccc}
\toprule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Pretrained}}} &
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Gauss FT}}} &  
\multirow{4}{*}{\textbf{Depth net}} & 
\multirow{4}{*}{\textbf{3D detector}} &
\multicolumn{6}{c}{Depth} &
\multicolumn{6}{c}{3D Detection}\vspace{0.5mm}\\
& 
&
&
&
\multicolumn{3}{c}{KITTI3D Train} & 
\multicolumn{3}{c}{KITTI3D Val} & 
\multicolumn{3}{c}{BEV AP} &
\multicolumn{3}{c}{3D AP}\\ 
&
&
& 
&
\multirow{2}{*}{Abs Rel$\downarrow$} &
\multirow{2}{*}{Sq Rel$\downarrow$} &
\multirow{2}{*}{RMSE$\downarrow$}&
\multirow{2}{*}{Abs Rel$\downarrow$} &
\multirow{2}{*}{Sq Rel$\downarrow$} &
\multirow{2}{*}{RMSE$\downarrow$}&
\multirow{2}{*}{Easy$\uparrow$} & 
\multirow{2}{*}{Med$\uparrow$}& 
\multirow{2}{*}{Hard$\uparrow$} &
\multirow{2}{*}{Easy$\uparrow$} & 
\multirow{2}{*}{Med$\uparrow$} & 
\multirow{2}{*}{Hard$\uparrow$} \vspace{0.0mm}\\
& & & & & & & & & & & & & & & \\
\midrule
& 
&
&
\multicolumn{12}{c}{Depth metrics computed on all Velodyne points.} \\
\midrule
&
& 
PackNet~\cite{guizilini20203d}  & 
Ours PL &
0.116 &	
0.844 & 
5.139 &	
0.112 & 
0.761 &
4.756 &
25.42 &	
17.97 &	
15.22 &  
18.50 & 
12.68 & 
10.78 \\


\checkmark &
& 
PackNet~\cite{guizilini20203d}  & 
Ours PL &
0.083 &
0.590 & 
3.839 &
0.079 &
0.489 &
3.577 &
41.59 &
27.75 &
23.69 &
30.91 &
20.53 &
17.25 \\

\midrule

&
&
BTS~\cite{lee2019big} & 
Ours PL &
0.100 &
0.635 &
4.479 & 
0.095 &
0.547 &
4.087 &
31.90 &
22.14 &
19.24 &
22.75 &
15.61 &
13.34 \\

\checkmark &
&
BTS~\cite{lee2019big} & 
Ours PL &
XXX &
XXX &
XXX & 
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX \\


\midrule

&
&
 -- & 
Ours FCOS &
XXX &
XXX &
XXX & 
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX \\

\checkmark &
&
 -- & 
Ours FCOS &
XXX &
XXX &
XXX & 
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX &
XXX \\
\midrule
&
&
& 
\multicolumn{12}{c}{Depth metrics computed on object Velodyne points (see Sec. 15.7).} \\
\midrule

&
& 
PackNet~\cite{guizilini20203d}  & 
Ours PL &
0.165 & 
1.257 & 
4.564 &	
0.176 &	
1.363 &	
4.883 &
25.42 &	
17.97 &	
15.22 &  
18.50 & 
12.68 & 
10.78 \\

% &
% \checkmark & 
% PackNet~\cite{guizilini20203d}  & 
% Ours PL &
% 0.159 &	
% 1.191 &	
% 4.433 &	
% 0.172 &	
% 1.317 &	
% 4.818 &
% 26.51 & 
% 18.64 &
% 16.00 &
% 18.97 &
% 13.09 &	
% 11.60 \\

\checkmark &
& 
PackNet~\cite{guizilini20203d}  & 
Ours PL &
0.115 &	
1.222 &	
3.658 &
0.111 &	
0.901 &
3.435 &
41.59 &
27.75 &
23.69 &
30.91 &
20.53 &
17.25 \\

\checkmark &
\checkmark & 
PackNet~\cite{guizilini20203d}  & 
Ours PL &
0.113 &	
0.801 &
3.337 &
0.112 &	
0.697 &	
3.301 &
43.46 & 
29.96 &
25.07 &
34.01 &
22.31 &
18.58 \\


\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{3D detection performance on the KITTI3D dataset with different depth inputs and different 3D detector architectures.}}
\label{table:ablation_depth_detection}
}
\end{table*}

==> tables/baseline_depth_detection.tex <==

\begin{table}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.5em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{Depth metrics} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Depth net} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$&
Easy$\uparrow$ & Med$\uparrow$ & Hard$\uparrow$ \vspace{0.5mm}\\
\midrule
PackNet~\cite{guizilini20203d}  & 
0.112 & 
0.761 &  
4.756 &  
18.50 &  
12.68 &  
10.78 \\
% BTS~\cite{lee2019big} & 
% 0.116 & 
% 0.935 &  
% 0.210 &  
% 0.842 &  
% 0.945 &  
% \textbf{0.977}\\
PSMNet~\cite{chang2018pyramid} & 
0.043 & 
0.390 &  
2.861 &  
64.83 &  
42.74 &  
34.75\\

\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{3D detection performance on the KITTI3D dataset~\cite{geiger2012we} with different depth inputs.} Packnet~\cite{guizilini20203d} computes depth from monocular images, while PSMNet~\cite{chang2018pyramid} computes depth from stereo. The depth metrics are computed against Velodyne lidar scans on the KITTI3D validation set. The 3D detection numbers are computed using the $AP|_{40}$ metric on the \textit{Car} category of the KITTI3D validation set.}
\label{table:baseline_depth_detection}
}
\end{table}

==> tables/cityscapes_results.tex <==

% \begin{table*}[t!]
% \centering
% {
% \footnotesize
% \setlength{\tabcolsep}{1em}
% \rowcolors{2}{lightgray}{white}
% \begin{tabular}{l|ccccccc|ccc}
% \toprule
% & \multicolumn{6}{c}{Detection Score (DS)} &  &  &  \\

% \multirow{-2}{*}{Method}& car & truck & bus & train & motorcycle & bicycle & mean & 
% \multirow{-2}{*}{AP} & \multirow{-2}{*}{BEV} & \multirow{-2}{*}{OS Yaw} \vspace{0.5mm}\\


% % 0.5m & 1.0m & 2.0m & 4.0m & 0.5m & 1.0m & 2.0m & 4.0m & 0.5m & 1.0m & 2.0m & 4.0m\\

% \midrule
% 3D-GSK~\cite{gahlert2020single} &
% 67.5 & 29.0 & 32.3 & 23.1 & 32.9 & 39.9 &	37.4 & 42.5 &	96.1 & 81.9 \\

% FCOS-3D &
% - & - & - & - & - & - & - & - & - & - \\

% % \bottomrule
% \end{tabular}\\\vspace{0mm}
% \caption{
% \textbf{FCOS 3D detection results on the nuScenes~\cite{caesar2020nuscenes} test set:} we report detailed results on the \textit{Car}, \textit{Pedestrian} and \textit{Bicycle} classes; detailed results for the other classes can be found in the supplementary.}
% \label{table:cityscapes_test_results}
% }
% \end{table*}



\begin{table}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{1.3em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|cccc}
\toprule
& DS & AP  & BEV  & OS Yaw  \\
% 0.5m & 1.0m & 2.0m & 4.0m & 0.5m & 1.0m & 2.0m & 4.0m & 0.5m & 1.0m & 2.0m & 4.0m\\

\midrule
3D-GSK~\cite{gahlert2020single} &
37.4 & 42.5 &	96.1 & 81.9 \\

FCOS-3D &
- & - & - & - \\



% \bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{FCOS 3D detection results on the CityScapes3D~\cite{gahlert2020cityscapes} test set:} we report detailed results on all the classes in the supplementary.}
\label{table:cityscapes_test_results}
}
\end{table}

==> tables/cs_nusc.tex <==

\begin{table*}[!h]
\centering
{
\footnotesize
\setlength{\tabcolsep}{1em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|cccccc|c}
\toprule
& \multicolumn{7}{c}{mAP} \\

\multirow{-2}{*}{Method}& 
Car & Bicycle & Motorcycle & Truck & Train & Bus & Mean\vspace{0.5mm}\\
\toprule
FCOS-3D (COCO) & 
37.27 &
18.58 &
11.89 &
5.77  &
1.43  &
11.33 &
14.38 \\
FCOS-3D (25K) & 
\textbf{43.97}  & 
\textbf{34.66}  & 
\textbf{23.19}  & 
\textbf{11.27}  & 
\textbf{5.49}  & 
\textbf{16.70} & 
\textbf{22.55} \\  

% \bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{Effect of depth pre-training on Cityscapes 3D.} Starting from the initial set of parameters trained on 2D detection task using MS-COCO dataset \cite{lin2014microsoft}, we measure the effect of additional pre-training on supervised depth prediction. The second stage pre-training significantly improves accuracy on \emph{all} categories, yielding a relative $\textbf{56.8\%}$ gain in \emph{mean AP}. 
%\textbf{FCOS 3D detection results on the CityScapes3D~\cite{gahlert2020cityscapes} validation set.}
\label{table:supp_cityscapes_val_results}
}
}
\end{table*}

==> tables/depth_vs_det2d.tex <==
%using the AP$|_{R_{40}}$ metric
%\textbf{Bold} denotes the best method, with \underline{underline} denoting the second best.
%using the AP$|_{R_{40}}$ metric
%\textbf{Bold} denotes the best method, with \underline{underline} denoting the second best.



\begin{table}[h]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Pre-train task}& 
Car & 
Ped. &
Cyclist &
Car & Ped. & Cyclist \vspace{0.5mm}\\
\midrule
2D-det (COCO~\cite{lin2014microsoft})  & 
20.24 & 
7.82 &
3.77 &
13.94 &
6.01 &
3.13
\\
\midrule
+ 2D-det (nuScenes~\cite{caesar2020nuscenes}) & 
20.45 & 
7.88 &
3.79 &
13.96 &
5.99 &
3.04
\\
+ Depth  (nuScenes~\cite{caesar2020nuscenes}) & 
\textbf{21.80} & 
\textbf{8.47} &
\textbf{3.81} &
\textbf{15.21} &
\textbf{6.61} &
\textbf{3.26}
\\
\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{\textbf{Depth vs. 2D detection as pre-training task.} We ablate the role of depth-pretraining, using a common set of images that are annotated both with 2D bounding boxes and (projected) 3D point-cloud.
\label{table:pretraining_depth_vs_detection}
}
}
\end{table}



==> tables/fcos_multitask.tex <==

\begin{table}[h]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.35em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Method}& 
Car & 
Ped. &
Cyclist &
Car & Ped. & Cyclist \vspace{0.5mm}\\
\midrule



FCOS-3D & 
25.82 & 
9.93&
4.36&
18.20 &
7.64 &
%3.75
3.76
\\

FCOS-3D Multi-task & 
%26.23 &
26.27 &
10.09&
3.91&
18.21 &
8.18 &
2.99
\\


\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{\textbf{Ablative analysis on different FCOS-3D fine-tuning strategies on the target dataset.} We present results when fine-tuning on the downstream task of 3D detection compared to a multi-task fine-tuning strategy that combines depth and 3D detection. The metrics are computed on the KITTI3D~\cite{geiger2012we} validation split.}
\label{table:fcos_multitask}
}
\end{table}


==> tables/kitti3d_test_multi_class.tex <==

\begin{table}[t]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{Pedestrian} & \multicolumn{3}{c}{Cyclist} \\ 
\multirow{-2}{*}{Methods}& 
Easy & 
Med &
Hard &
Easy & Med & Hard \vspace{0.5mm}\\
\midrule
OFTNet~\cite{} &
1.28 &
0.81 &
0.51 &
0.36 &
0.16 &
0.15 
\\
SS3D~\cite{} &
2.48 &
2.09 &
1.61 &
3.45 &
1.89 &
1.44 
\\
M3D-RPN~\cite{} &
5.65 &
4.05 &
3.29 &
1.25 &
0.81 &
0.78 
\\
MonoPSR~\cite{} &
7.24 &
4.56 &
4.11 &
\textbf{9.87} &
\textbf{5.78} &
\textbf{4.57} 
\\
MonoDIS (multi)~\cite{simonelli2020disentangling} & 
9.07 & 
5.81 &
5.09 &
1.47 &
0.85 &
0.61
\\
\midrule
DD3D & 
\textbf{15.86} & 
\textbf{10.49} &
\textbf{9.06} &
5.00 &
3.06 &
2.56
\\
\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{KITTI-3D benchmark evaluation on \emph{Pedestrian} and \emph{Cyclist}.}
%Multiclass 3D detection on the KITTI3D test set. We report BEV and 3D AP$|_{R_{40}}$ metrics for "Pedestrian" and "Cyclist" category. DD3D outperforms most of other approaches, with \textbf{80.5\%} improvement from the previous best method on "Pedestrian". 
}
\label{table:kitti_3d_test_multi_class}
}
\end{table}

==> tables/kitti3d_val.tex <==

\begin{table}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Methods}& 
Easy & 
Med &
Hard &
Easy & Med & Hard \vspace{0.5mm}\\
\midrule
% ROI-10D~\cite{manhardt2019roi} & 
% 9.78 & 
% 4.91 &
% 3.74 &
% 4.32 &
% 2.02 &
% 1.46
% \\
% GS3D~\cite{li2019gs3d} & 
% 8.41 & 
% 6.08 &
% 4.94 &
% 4.47 &
% 2.90 &
% 2.47
% \\
MonoGRNet~\cite{qin2019monogrnet} & 
19.72 & 
12.81 &
10.15 &
11.90 &
7.56 &
5.76
\\

% MonoPSR~\cite{ku2019monocular} & 
% 18.33 & 
% 12.58 &
% 9.91 &
% 10.76 &
% 7.25 &
% 5.85
% \\

% SS3D~\cite{jorgensen2019monocular} & 
% 16.33 & 
% 11.52 &
% 9.93 &
% 10.78 &
% 7.68 &
% 6.51
% \\

MonoDIS (single)~\cite{simonelli2019disentangling} & 
18.45 & 
12.58 &
10.66 &
11.06 &
7.60 &
6.37
\\

M3D-RPN~\cite{brazil2019m3d} & 
20.85 & 
15.62 &
11.88 &
14.53 &
11.07 &
8.65
\\

% SMOKE~\cite{liu2020smoke} & 
% 20.83 & 
% 14.49 &
% 12.75 &
% 14.03 &
% 9.76 &
% 7.84
% \\

MonoPair~\cite{chen2020monopair} & 
24.12 & 
18.17 &
15.76 &
16.28 &
12.30 &
10.42
\\

MonoDIS (multi)~\cite{simonelli2020disentangling} & 
23.40 & 
17.20 &
15.30 &
16.50 &
12.20 &
10.30
\\

Kinematic3D~\cite{brazil2020kinematic} & 
27.83 & 
19.72 &
15.10 &
19.76 &
14.10 &
10.47
\\

% \midrule
% \multicolumn{7}{c}{Baselines (no depth pre-training)}
% \\

% DD3D \tiny{(DLA34, COCO)} & 
% 26.77 &
% 20.24 &
% 16.72 &
% 18.84 &
% 13.94 &
% 11.25 
% \\

% DD3D \tiny{(V99, COCO)} & 
% 25.51 &
% 18.72 &
% 15.48 &
% 17.60 &
% 12.92 &
% 10.48 
% \\

% PL \tiny{(KITTI-depth)} & 
% 27.61 &	
% 19.19 &	
% 16.43 &  
% 18.11 & 
% 12.70 & 
% 10.63
% \\


\midrule

% \multicolumn{7}{c}{Depth pre-trained (2.5M-set)}
% \\

% DD3D \tiny{(DLA34, 2.5M)} & 
% % 32.02 &
% % 24.06 &
% % 20.42 &
% % 22.80 &
% % 17.03 &
% % 13.77 
% %33.23 &
% %25.82 &
% %21.75 &
% %24.01 &
% %18.20 &
% %14.85
% 31.66 &
% 23.96 &
% 20.31 &
% 21.94 &
% 16.45 &
% 13.55
% \\
% \quad + \scriptsize{COCO} &
% 33.45 &
% 26.01 &
% 22.55 &
% 24.11 &
% 18.37 &
% 15.42
% \\
PL &  
\textbf{43.51} & 
\textbf{30.06} &
\underline{25.37} &
\textbf{32.10} &
\textbf{22.36} &
\textbf{19.20} 
\\

DD3D &
\underline{36.96} &
\underline{29.42} &
\textbf{25.40} &
\underline{27.21} &
\underline{21.42} &
\underline{17.75}
\\




\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{3D detection performance on the KITTI3D validation set} for the \emph{Car} category. Baselines of DD3D denotes models that are fine-tuned from COCO-pretrained parameters. Baseline of Pseudo-Lidar method uses depth network trained on \emph{eigen-clean} set of KITTI-Depth dataset. Pre-training depth network with a large set of image-Lidar pairs brings significant improvement for both approaches. We report 3D Box AP$|_{R_{40}}$ metric.
\label{table:kitti_3d_val}
}
}
\end{table}

%using the AP$|_{R_{40}}$ metric
%\textbf{Bold} denotes the best method, with \underline{underline} denoting the second best.

==> tables/kitti_depth.tex <==

\begin{table}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|cccc}
\toprule
% \multirow{2}{*}{\textbf{Method}} &
% \multicolumn{3}{|c|}{Lower is better $\downarrow$} &
% \multicolumn{3}{|c}{Higher is better $\uparrow$} \\
Method & 
Abs.Rel$\downarrow$ &
Sqr.Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}\uparrow$ 
% a2 &
% a3
\\
\toprule

Kuznietsov et al. \cite{kuznietsov2017semi}
% & 0.113 & 0.741 & 4.621 & 0.862 & 0.960 & 0.986
& 0.113 & 0.741 & 4.621 & 0.862 
\\
Gan et al. \cite{Gan2018MonocularDE}
% & 0.098 & 0.666 & 3.933 & 0.890 & 0.964 & 0.985
& 0.098 & 0.666 & 3.933 & 0.890
\\
Guizilini et al. ~\cite{packnet-semisup}
% & 0.078 & 0.378 & 3.330 & 0.927 & --- & ---
& 0.078 & 0.378 & 3.330 & 0.927 
\\
Fu et al. \cite{fu2018deep}
% & 0.072 & 0.307 & 2.727 & 0.932 & 0.984 & 0.994
& 0.072 & 0.307 & 2.727 & 0.932
\\
Yin et al. \cite{Yin2019enforcing}
% & 0.072 & --- & 3.258 & 0.938 & 0.990 & 0.998
& 0.072 & --- & 3.258 & 0.938 
\\
Lee et al. ~\cite{lee2019big} 
% & 0.059 & 0.245 & 2.756 & 0.956 & 0.993 & 0.998
& 0.059 & 0.245 & 2.756 & 0.956
\\

\midrule

Ours PackNet 
% & 0.053 & 0.179 & 2.301 & 0.968 & 0.996 & 0.999
& 0.053 & 0.179 & 2.301 & 0.968
\\
Ours BTS
% & 0.051 & 0.166 & 2.234 & 0.972 & 0.996 & 0.999
& 0.051 & 0.166 & 2.234 & 0.972
\\

\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on the KITTI dataset}, for the \textit{Eigen} test split \cite{eigen2014depth} and distances up to 80m.} 
\label{table:depth_kitti}

\end{table}



==> tables/kitti_val_ablation.tex <==
% RA: This table should contain DD3D and PL baselines (no depth pretraining), final models and ablations with different backbones for DD3D

\begin{table}
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.6em}
\begin{tabular}{l|cc|ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} &
\multirow{2}{*}{Pre-train} & \multicolumn{3}{c}{BEV AP} \\
& & & 
Easy & 
Mod &
Hard \\
\midrule
\multicolumn{6}{c}{No large-scale depth pre-training} \\
\midrule
PL & PackNet & KITTI &
27.6 &	
19.2 &	
16.4 
\\
DD3D & DLA-34 & COCO &
26.8 &
20.2 &
16.7 
\\
DD3D & V2-99 & COCO & 
25.5 &
18.7 &
15.5 
\\
\midrule
\multicolumn{6}{c}{With large-scale depth pre-training} \\
\midrule
PL & PackNet & DDADv2 &
xx.x &
xx.x &
xx.x
\\
PL & PackNet & DDADv2 $\rightarrow$ KITTI &  
43.5 & 
30.1 &
25.4 
\\
DD3D  & DLA-34 & DDADv2 &
31.7 &
24.0 &
20.3 
\\
DD3D & DLA-34 & COCO $\rightarrow$ DDADv2 &
33.5 &
26.0 &
22.6 
\\
DD3D & V2-99 & COCO $\rightarrow$ DDADv2 &
37.0 &
29.4 &
25.4
\\
\bottomrule
\end{tabular}
\caption{\textbf{Ablating the effect of depth pre-training} from PL and DD3D using various backbones. As pre-training methods, KITTI denotes dense depth prediction using \emph{eigen} split of KITTI-Depth dataset, COCO denotes 2D detection using COCO train dataset, and DDADv2 denotes dense depth prediction using DDADv2 dataset. The right arrow ($\rightarrow$) denotes sequential pre-training phases. We report 3D BEV AP$|_{R_{40}}$ metrics on \emph{Car}. 
}
\label{table:kitti_3d_val}
}
\end{table}


\iffalse

\begin{table}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Methods}& 
Easy & 
Med &
Hard &
Easy & Med & Hard \vspace{0.5mm}\\
\midrule
\multicolumn{7}{c}{No large-scale depth pre-training}
\\
DD3D \scriptsize{(DLA34)} & 
26.77 &
20.24 &
16.72 &
18.84 &
13.94 &
11.25 
\\

DD3D \scriptsize{(V2-99)} & 
25.51 &
18.72 &
15.48 &
17.60 &
12.92 &
10.48 
\\

PL \scriptsize{(KITTI-depth)} & 
27.61 &	
19.19 &	
16.43 &  
18.11 & 
12.70 & 
10.63
\\


\midrule

\multicolumn{7}{c}{With large-scale depth pre-training}
\\

DD3D \tiny{(DLA34, 2.5M)} & 
31.66 &
23.96 &
20.31 &
21.94 &
16.45 &
13.55
\\
\quad + \scriptsize{COCO} &
33.45 &
26.01 &
22.55 &
24.11 &
18.37 &
15.42
\\
DD3D \tiny{(V99, COCO $\rightarrow$ 2.5M}) &
\underline{36.96} &
\underline{29.42} &
\textbf{25.40} &
\underline{27.21} &
\underline{21.42} &
\underline{17.75}
\\

PL \tiny{(2.5M $\rightarrow$ eigen-clean)} &  
\textbf{43.51} & 
\textbf{30.06} &
\underline{25.37} &
\textbf{32.10} &
\textbf{22.36} &
\textbf{19.20} 
\\


\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{3D detection performance on the KITTI3D validation set} for the \emph{Car} category. Baselines of DD3D denotes models that are fine-tuned from COCO-pretrained parameters. Baseline of Pseudo-Lidar method uses depth network trained on \emph{eigen-clean} set of KITTI-Depth dataset. Pre-training depth network with a large set of image-Lidar pairs brings significant improvement for both approaches. We report 3D Box AP$|_{R_{40}}$ metric.
}
\label{table:kitti_3d_val}
}
\end{table}

%using the AP$|_{R_{40}}$ metric
%\textbf{Bold} denotes the best method, with \underline{underline} denoting the second best.

\fi

==> tables/kitti_val_ablation_v2.tex <==



\begin{table}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{6}{c}{Car} \\
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Methods}& 
Easy & 
Med &
Hard &
Easy & Med & Hard \vspace{0.5mm}\\

\midrule

%MonoGRNet~\cite{qin2019monogrnet} & 
%19.72 & 
%12.81 &
%10.15 &
%11.90 &
%7.56 &
%5.76
%\\


MonoDIS (single)~\cite{simonelli2019disentangling} & 
18.45 & 
12.58 &
10.66 &
11.06 &
7.60 &
6.37
\\

M3D-RPN~\cite{brazil2019m3d} & 
20.85 & 
15.62 &
11.88 &
14.53 &
11.07 &
8.65
\\

MonoPair~\cite{chen2020monopair} & 
24.12 & 
18.17 &
15.76 &
16.28 &
12.30 &
10.42
\\

%MonoDIS (multi)~\cite{simonelli2020disentangling} & 
%23.40 & 
%17.20 &
%15.30 &
%16.50 &
%12.20 &
%10.30
%\\

Kinematic3D~\cite{brazil2020kinematic} & 
27.83 & 
19.72 &
15.10 &
19.76 &
14.10 &
10.47
\\

\midrule
\multicolumn{7}{c}{DD3D with V2-99 backbone} \\ 
\midrule

DD3D [V2-99] & 
36.96 &
29.42 &
25.40 &
27.21 &
21.42 &
17.75
\\


\quad $-$ DDAD15M & 
25.51 &
18.72 &
15.48 &
17.60 &
12.92 &
10.48 
\\



\midrule
\multicolumn{7}{c}{DD3D with DLA34 backbone} \\ 

\midrule

DD3D [DLA34] & 
33.45 &
26.01 &
22.55 &
24.11 &
18.37 &
15.42 
\\ 


\quad $-$ DDAD15M &
26.77 &
20.24 &
16.72 &
18.84 &
13.94 &
11.25 
\\

\quad $-$ COCO &
31.66 &
23.96 &
20.31 &
21.94 &
16.45 &
13.55
\\

\quad $+$ Multi-task & 
34.62 & 
26.27 &
22.12 &
24.12 &
18.21 &
14.89 
\\



\midrule
\multicolumn{7}{c}{Pseudo-Lidar} \\ 
\midrule

PL &  
43.51 & 
30.06 &
25.37 &
32.10 &
22.36 &
19.20 
\\

\quad $-$ KITTI Finetune &  
25.82 & 
19.09 &
16.35 &
18.23 &
13.32 &
11.59 
\\

\quad $-$ DDAD15M &  
27.61 &	
19.19 &	
16.43 &  
18.11 & 
12.70 & 
10.63 
\\


\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{Ablative analysis of 3D detection performance of DD3D and PL on the KITTI-3D validation set} for the \emph{Car} category. Please refer to Section~\ref{subsec:ablative} for a detailed discussion of the results.
\label{table:kitti_3d_val_ablation}
}
}
\end{table}

%using the AP$|_{R_{40}}$ metric
%\textbf{Bold} denotes the best method, with \underline{underline} denoting the second best.

==> tables/nuscenes_all.tex <==

\begin{table*}
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.4em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
& \multicolumn{4}{c}{PointPillars~\cite{lang2019pointpillars}}& \multicolumn{4}{c}{MonoDis~\cite{simonelli2020demystifying}}& \multicolumn{4}{c}{FCOS-3D} \\

\multirow{-2}{*}{Category}& 
AP[\%]$\uparrow$ & ATE$\downarrow$ & ASE[1-IoU]$\downarrow$ & AOE[rad]$\downarrow$ &
AP[\%]$\uparrow$ & ATE$\downarrow$ & ASE[1-IoU]$\downarrow$ & AOE[rad]$\downarrow$ &
AP[\%]$\uparrow$ & ATE$\downarrow$ & ASE[1-IoU]$\downarrow$ & AOE[rad]$\downarrow$\vspace{0.5mm}\\

\midrule

Barrier & 39.0  & 0.71 & 0.30 & \textbf{0.08} & 50.0  & 0.54 & 0.28 & 0.22 &  \textbf{52.9} & \textbf{0.50} & \textbf{0.27} & 0.12 \\
Bicycle & 1.0  & \textbf{0.31} & 0.32 & \textbf{0.54} & 25.0 & 0.68 & \textbf{0.29} & 1.25  & \textbf{26.9} & 0.63 & 0.31 &  0.97  \\
Bus & \textbf{28.0}  & \textbf{0.56} & \textbf{0.20} & 0.25 & 15.0 & 0.85 & \textbf{0.20} & 0.12 & 16.0 & 0.93 &  \textbf{0.20} & \textbf{0.07} \\
Car & \textbf{68.0}  & \textbf{0.28} & 0.16 & 0.20 & 46.0 & 0.62 & \textbf{0.15} & 0.08 & 54.9 & 0.49 & \textbf{0.15} & \textbf{0.07} \\
Constr.Veh. & 4.0  & \textbf{0.89} & 0.49 & 1.26 &  6.0 & 1.02 & 0.41 & 1.05 & \textbf{10.1} & 0.97 & \textbf{0.39} & \textbf{0.94}  \\
Motorcycle & 27.0  & \textbf{0.36} & 0.29 & 0.79 &  30.0 & 0.70 & \textbf{0.24} & 0.57  & \textbf{30.9} &  0.64 & 0.25 & \textbf{0.48}  \\
Pedestrian & \textbf{60.0}  & \textbf{0.28} & 0.31 & \textbf{0.37} &  36.0 & 0.69 & \textbf{0.30} & 1.46  & 42.4 &  0.66 & 0.31 &  0.75  \\
Traffic Cone & 31.0  & \textbf{0.40} & 0.39 & - & 49.0 & 0.49 & \textbf{0.33} & – & \textbf{55.3} &  0.44 & 0.35 & -  \\
Trailer & \textbf{23.0}  & 0.89 & \textbf{0.20} & 0.83 &  16.0 & 1.03 & \textbf{0.20} & 0.78  & 17.4 & \textbf{0.88} & \textbf{0.20} & \textbf{0.72}  \\
Truck  & 23.0  & \textbf{0.49} & 0.23 & 0.18 &  21.0 & 0.79 & 0.20 & 0.10  & \textbf{23.5} & 0.68 & \textbf{0.19} & \textbf{0.07}  \\
\midrule
\textbf{Mean} & 31.0 & \textbf{0.52} & 0.29 & 0.50 & 30.0  & 0.74 & \textbf{0.26} & 0.62 & \textbf{33.0} & 0.68 &  \textbf{0.26} & \textbf{0.47} \\
\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{\textbf{Results on nuScenes \emph{test}.} In addition to \emph{average precision}, FCOS-3D generally outperforms the previous best vision-based algorithm (\textbf{MonoDIS}) and a widely used Lidar-based algorithm (\textbf{PointPillars}) on multi-class metrics relevant to 3D detection. FCOS-3D is particularly robust in detecting rare objects, such as \emph{Construction Vehicle} and \emph{Traffic Cone}.}
%\textbf{FCOS 3D detailed detection results on the nuScenes~\cite{caesar2020nuscenes} test set.}}
\label{table:supp_nuscenes_all}
}
\end{table*}

% \begin{table*}
% \centering
% {
% \footnotesize
% \setlength{\tabcolsep}{0.4em}
% \rowcolors{2}{lightgray}{white}
% \begin{tabular}{l|cccc|cccc}
% \toprule
% & \multicolumn{4}{c}{MonoDis~\cite{simonelli2020demystifying}}& \multicolumn{4}{c}{FCOS-3D} \\
%
% \multirow{-2}{*}{Category}& 
% AP[\%]$\uparrow$ & ATE$\downarrow$ & ASE[1-IoU]$\downarrow$ & AOE[rad]$\downarrow$ &
% AP[\%]$\uparrow$ & ATE$\downarrow$ & ASE[1-IoU]$\downarrow$ & AOE[rad]$\downarrow$\vspace{0.5mm}\\
% 
% \midrule
% 
% Barrier & 50.0  & 0.54 & 0.28 & 0.22 &  52.9 & 0.50 & 0.27 & 0.12 \\
% Bicycle & 25.0 & 0.68 & 0.29 & 1.25  & 26.9 & 0.63 & 0.31 &  0.97  \\
% Bus & 15.0 & 0.85 & 0.20 & 0.12 & 16.0 & 0.93 &  0.20 & 0.07 \\
% Car & 46.0 & 0.62 & 0.15 & 0.08 & 54.9 & 0.49 & 0.15 & 0.07 \\
% Constr.veh. &  6.0 & 1.02 & 0.41 & 1.05 &  & 0.97 & 0.39 & 0.94  \\
% Motorcycle &  30.0 & 0.70 & 0.24 & 0.57  & 30.9 &  0.64 & 0.25 & 0.48  \\
% Pedestrian &  36.0 & 0.69 & 0.30 & 1.46  & 42.4 &  0.66 & 0.31 &  0.75  \\
% Traffic\_cone & 49.0 & 0.49 & 0.33 & – & 55.3 &  0.44 & 0.35 & -  \\
% Trailer &  16.0 & 1.03 & 0.20 & 0.78  & 17.4 & 0.88 & 0.20 & 0.72  \\
% Truck  &  21.0 & 0.79 & 0.20 & 0.10  & 23.5 & 0.68 & 0.19 & 0.07  \\
% Mean & 30.0  & 0.74 & 0.26 & 0.62 & - & 13.0  & 33.0 &  0.68 &  0.26 & 0.47 &  1.69 & 1.0 \\
% \bottomrule
% \end{tabular}\\\vspace{0mm}
% \caption{
% \textbf{FCOS 3D detailed detection results on the nuScenes~\cite{caesar2020nuscenes} test set.}}
% \label{table:supp_nuscenes_all}
% }
% \end{table*}


% \begin{table*}
% \centering
% {
% \footnotesize
% \setlength{\tabcolsep}{0.4em}
% \rowcolors{2}{lightgray}{white}
% \begin{tabular}{l|cccccc|cccccc}
% \toprule
% & \multicolumn{6}{c}{MonoDis~\cite{simonelli2020demystifying}}& \multicolumn{6}{c}{FCOS-3D} \\

% \multirow{-2}{*}{Category}& 
% AP[\%]$\uparrow$ & ATE$\downarrow$ & ASE[1-IoU]$\downarrow$ & AOE[rad]$\downarrow$ & AVE[m]$\downarrow$ & AAE[\%]$\downarrow$  & 
% AP[\%]$\uparrow$ & ATE$\downarrow$ & ASE[1-IoU]$\downarrow$ & AOE[rad]$\downarrow$ & AVE[m]$\downarrow$ & AAE[\%]$\downarrow$\vspace{0.5mm}\\

% \midrule

% Barrier & 50.0  & 0.54 & 0.28 & 0.22 & - & – &  52.9 & 0.50 & 0.27 & 0.12 & - & - \\
% Bicycle & 25.0 & 0.68 & 0.29 & 1.25 & - & 1.0 & 26.9 & 0.63 & 0.31 &  0.97 & 0.91 &  1.0 \\
% Bus & 15.0 & 0.85 & 0.20 & 0.12 & - & 32.0 & 16.0 & 0.93 &  0.20 & 0.07 & 3.10 &  1.0 \\
% Car & 46.0 & 0.62 & 0.15 & 0.08 & - & 12.0 & 54.9 & 0.49 & 0.15 & 0.07 & 1.79 & 1.0 \\
% Constr.veh. &  6.0 & 1.02 & 0.41 & 1.05 & - & 9.0 & 10.1  & 0.97 & 0.39 & 0.94 &  0.53 & 1.0 \\
% Motorcycle &  30.0 & 0.70 & 0.24 & 0.57 & - & 1.0 & 30.9 &  0.64 & 0.25 & 0.48 & 3.35 & 1.0 \\
% Pedestrian &  36.0 & 0.69 & 0.30 & 1.46 & - & 18.0 & 42.4 &  0.66 & 0.31 &  0.75 & 0.89 &  1.0 \\
% Traffic\_cone & 49.0 & 0.49 & 0.33 & – & - & – & 55.3 &  0.44 & 0.35 & - & - & - \\
% Trailer &  16.0 & 1.03 & 0.20 & 0.78 & - & 11.0 & 17.4 & 0.88 & 0.20 & 0.72 &  0.87 & 1.0 \\
% Truck  &  21.0 & 0.79 & 0.20 & 0.10 & - & 16.0 & 23.5 & 0.68 & 0.19 & 0.07 & 2.04 & 1.0 \\
% % Mean & 30.0  & 0.74 & 0.26 & 0.62 & - & 13.0  & 33.0 &  0.68 &  0.26 & 0.47 &  1.69 & 1.0 \\
% % \bottomrule
% \end{tabular}\\\vspace{0mm}
% \caption{
% \textbf{FCOS 3D detailed detection results on the nuScenes~\cite{caesar2020nuscenes} test set.}}
% \label{table:supp_nuscenes_all}
% }
% \end{table*}




==> tables/nuscenes_per_class.tex <==

\begin{table}[!h]
\centering
{
\footnotesize
\setlength{\tabcolsep}{1em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|cccc}
\toprule
& \multicolumn{4}{c}{AP [\%] $\uparrow$} \\

\multirow{-2}{*}{Category}& 
0.5m & 1.0m & 2.0m & 4.0m \vspace{0.5mm}\\

\toprule
Barrier &
18.8 &
52.2 &
67.9 &
72.2 \\
Bicycle &
6.9  &
22.6 &
35.4 &
42.7 \\
Bus &
0.0 & 
3.6 &
23.2 &
37.3 \\
Car &
19.6 &
47.1 &
71.2 &
81.5 \\
Construction\_vehicle & 
0.0 &
1.9 &
13.5 &
25.0 \\
Motorcycle &
7.0 &
26.2 &
41.8 &
48.5 \\
Pedestrian & 
12.5 &
35.0 &
55.4 &
66.5 \\
Traffic\_cone &
31.7 &
53.3 &
64.8 &
71.3 \\
Trailer &
0.0 &
5.4 &
23.4 &
40.7 \\
Truck &
2.8 &
15.8 &
32.5 &
43.0 \\

% \bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{FCOS 3D detection results on the nuScenes~\cite{caesar2020nuscenes} test set:} detailed results for the AP metrics on all classes.}
\label{table:supp_nuscenes_per_class}
}
\end{table}

==> tables/pl_data_vs_det.tex <==

\begin{table}[h!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.5em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{Data split} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Depth net} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$&
Easy$\uparrow$ & Med$\uparrow$ & Hard$\uparrow$ \vspace{0.5mm}\\
\midrule

\textbf{Scratch}  & 
0.112 & 
0.761 &  
4.756 &  
18.11 &  
12.70 &  
10.63 \\

 \textbf{1K}  & 
0.101 & 
0.560 &  
3.891 &  
22.13 &  
15.05 &  
13.00 \\

\textbf{5K}  & 
0.093 & 
0.505 &  
3.692 &  
28.86 &  
18.88 &  
15.67 \\

\textbf{10K}  & 
0.091 & 
0.501 &  
3.722 &  
27.35 &  
18.41 &  
15.25 \\

\textbf{25K}  & 
0.079 & 
0.489 &  
3.577 &  
32.10 &  
22.36 &  
19.20 \\

\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
%\textbf{3D detection accuracy on the KITTI3D~\cite{geiger2012we} validation split with different depth inputs.} 
\textbf{How accurate does the depth predictor need to be for the Pseudo-Lidar detector?} We train a PackNet~\cite{guizilini20203d} depth estimator with increasing amounts of training data, subsequently fine-tuned on the KITTI3D Eigen clean split. We generate depth maps from each depth network on the KITTI3D train and validation splits, and train a Pseudo-Lidar 3D detector using predicted depth as input. We report $AP|_{40}$ metric on the \textit{Car} class. Both 3D and depth metrics are computed on the KITTI3D \emph{val} set. Note that this table complements Fig. 4 in the main paper.}
\label{table:supp_pl_data_vs_det}
}
\end{table}



==> tables/results_multi_task.tex <==

\begin{table*}
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.35em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc||ccc|ccc||ccc|ccc}
\toprule
& \multicolumn{6}{c}{Car} & \multicolumn{6}{c}{Pedestrian} & \multicolumn{6}{c}{Cyclist} \\
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} & \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} & \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-3}{*}{Method}& 
Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\vspace{0.5mm} \\
\toprule
FCOS-3D & 
33.23 & 25.82 & 21.75 & 24.01 & 18.20 & 14.85 &
12.58 & 9.93&  \textbf{7.88} & 9.76 & 7.64 & 5.80 & 
\textbf{7.58} & \textbf{4.36} & \textbf{3.64} & \textbf{6.60} & \textbf{3.76} & \textbf{2.98} \\




FCOS-3D Multi-task & 
\textbf{34.62} & \textbf{26.27} & \textbf{22.12} & \textbf{24.12} & \textbf{18.21} & \textbf{14.89} &
\textbf{12.79} & \textbf{10.09} &  7.77 & \textbf{10.51} & \textbf{8.18} & \textbf{6.05} & 
6.58 & 3.91& 3.17 & 5.14 & 2.99 & 2.41 \\



\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{
\textbf{Supervised depth prediction as auxiliary task during fine-tuning.} We present the full experimental results showing the effect of using region-of-interest (RoI) focused depth supervision as an auxiliary task during fine-tuning for 3D detection. This complements Table 8 of the main paper by including "Easy" and "Hard" metrics of KITTI-3D benchmark.
%\textbf{Ablative analysis on different FCOS-3D fine-tuning strategies on the target dataset.} We present detailed results using the BeV and 3DAP metrics, complementing the results from Table 8 in the main submission. The metrics are computed on the KITTI3D~\cite{geiger2012we} validation split.
}
\label{table:supp_detailed_multi_task}
}
\end{table*}


==> tables/v2_99.tex <==

\begin{table}[t!]
\centering
{
\footnotesize
\setlength{\tabcolsep}{0.2em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
\multirow{-2}{*}{Backbone}& 
Car & 
Pedestrian &
Cyclist &
Car & Pedestrian & Cyclist \vspace{0.5mm}\\
\midrule

V2-99 \cite{lee2019centermask} & 
8.40 & 
2.49 &
0.09 &
4.58 &
1.70 &
0.03
\\

DLA-34~\cite{yu2018deep}  & 
20.24 & 
7.82 &
3.77 &
13.94 &
6.01 &
3.13
\\

\midrule



V2-99 \cite{lee2019centermask} + 25K & 
24.27 & 
9.59 &
3.34 &
17.34 &
\textbf{8.17} &
2.65
\\

DLA-34~\cite{yu2018deep} + 25K & 
\textbf{25.82} & 
\textbf{9.93} &
\textbf{4.36} &
\textbf{18.20} &
7.64 &
\textbf{3.75}
\\

\bottomrule
\end{tabular}\\\vspace{0mm}
\caption{\textbf{Alternative backbones for FCOS-3D:} we show results with the DLA-34~\cite{yu2018deep} and V2-99 \cite{lee2019centermask} networks. All networks are fine-tuned for 3D detection on the KITTI3D~\cite{geiger2012we} train split and the metrics are computed on KITTI3D val split. \textit{+ 25K} denotes additional monocular depth pre-training on the 25K split (2.5M images).}
\label{table:v2-99}
}
\end{table}



% \begin{table}[t!]
% \centering
% {
% \footnotesize
% \setlength{\tabcolsep}{0.4em}
% \rowcolors{2}{lightgray}{white}
% \begin{tabular}{c|ccc|ccc}
% \toprule
% & \multicolumn{3}{c}{BEV AP} & \multicolumn{3}{c}{3D AP} \\ 
% \multirow{-2}{*}{Pre-train task}& 
% Car & 
% Pedestrian &
% Cyclist &
% Car & Pedestrian & Cyclist \vspace{0.5mm}\\
% \midrule
% %  DLA-34, Det2D & 
% % 16.84 & 
% % 7.01 &
% % 2.88 &
% % 11.20 &
% % 5.64 &
% % 2.40
% % \\
% 2D Det. (coco)  & 
% 8.40 & 
% 2.49 &
% 0.09 &
% 4.58 &
% 1.70 &
% 0.03
% \\

%   + Depth & 
% \textbf{24.27} & 
% \textbf{9.59} &
% \textbf{3.34} &
% \textbf{17.34} &
% \textbf{8.17} &
% \textbf{2.65}
% \\
% \bottomrule
% \end{tabular}\\\vspace{0mm}
% \caption{Ablative analysis on using different backbones for FCOS-3D.}
% \label{table:v2-99}
% }
% \end{table}

% % Pre-training on supervised depth estimation allows for training larger backbone of FCOS-3D. We pre-train V2-99 \cite{lee2019centermask} backbone (96.9M parameters) using 2D detection on MS-COCO dataset, and perform additional pre-training using depth prediction on our internal dataset of image-pointcloud pairs. The models are then fine-tuned on KITTI \emph{train} for 3D detection, and evaluated on KITTI \emph{val}. The depth pre-training significantly improve rare classes: 4$\times$ for "Pedestrian", 37$\times$ for "Cyclist". We run each fine-tuning experiment four times, and report the average. We only report "Moderate" metrics due to limited space.
